Sparse Decomposition of Graph Neural Networks

Graph Neural Networks (GNN) exhibit superior performance in graph representation learning, but their inference cost can be high, due to an aggregation operation that can require a memory fetch for a very large number of nodes. This inference cost is the major obstacle to deploying GNN models with \emph{online prediction} to reflect the potentially dynamic node features. To address this, we propose an approach to reduce the number of nodes that are included during aggregation. We achieve this through a sparse decomposition, learning to approximate node representations using a weighted sum of linearly transformed features of a carefully selected subset of nodes within the extended neighbourhood. The approach achieves linear complexity with respect to the average node degree and the number of layers in the graph neural network. We introduce an algorithm to compute the optimal parameters for the sparse decomposition, ensuring an accurate approximation of the original GNN model, and present effective strategies to reduce the training time and improve the learning process. We demonstrate via extensive experiments that our method outperforms other baselines designed for inference speedup, achieving significant accuracy gains with comparable inference times for both node classification and spatio-temporal forecasting tasks.

==> Makefile <==
# Makefile for LaTeX document files
# Created: July 3, 2015. Last modified: Apr. 25, 2023.

# Set up the paths and names
# Default output is named "main". Default section path "./sections". Default figure path "./figures"
DOCUMENT=main
SECPATH=sections/
FIGPATH=figures/
LATEX=pdflatex --shell-escape

SECTIONS=$(wildcard $(SECPATH)*.tex)
FIGURES=$(wildcard $(FIGPATH)*.pdf)

$(DOCUMENT).pdf : $(DOCUMENT).tex $(SECTIONS) $(FIGURES) $(DOCUMENT).aux 
	$(LATEX)  $(DOCUMENT).tex

# for blocks of figures
$(FIGPATH)%.pdf : $(FIGPATH)%.eps 
	epstopdf $
# $(FIGPATH)%.pdf : $(FIGPATH)%.svg
# 	inkscape --export-filename=$@ $<

$(DOCUMENT).aux : $(DOCUMENT).bib
	$(LATEX)  $(DOCUMENT).tex
	bibtex $(DOCUMENT)
	$(LATEX)  $(DOCUMENT).tex

all : 
	$(LATEX)  $(DOCUMENT).tex
	bibtex $(DOCUMENT)
	$(LATEX)  $(DOCUMENT).tex
	$(LATEX)  $(DOCUMENT).tex

clean:
	rm -rf *.aux $(DOCUMENT).log $(DOCUMENT).toc $(DOCUMENT).dvi \
    $(DOCUMENT).pdf $(DOCUMENT).bbl $(DOCUMENT).blg \
    $(DOCUMENT).out



==> TODO.tex <==
%!TEX root = /Users/yaochen/Dropbox/Apps/Overleaf/AAAI25-SDGNN/main.tex
% Getting things done
{\bf TODO:}
\begin{enumerate}
    \item think about the expressive power proof. 
    \item LARS parameter tuning about the threshold.
\end{enumerate}

\begin{enumerate}
    \item Fix PPRGo results
\end{enumerate}
\newpage
\setcounter{page}{1}






==> sections/analysis.tex <==
%!TEX root = /Users/yaochen/Dropbox/Apps/Overleaf/TMLR25-SDGNN/main.tex
\section{Analysis}

Let $M(\rmX; \rmW):\mathbb{R}^{|\gV|\times D\rightarrow |\gV|\times D^\prime}$ be the function that generates a matrix results by applying row-wise MLP on the input matrix $\rmX$, where $\rmW$ is the parameters in MLP. 

Define 
\begin{align}
    & g_1(\rmX) = M(\rmA\rmX, \rmW_1),\\
    & g_k(\rmX) = M(\rmA g_{k-1}(\rmX), \rmW_k), \quad \forall k=2,\ldots,
\end{align}
where $g_k(\rmX)$ can represent most of GNN models with $k$-layers. Define
\begin{align}
    f(\rmX) = \rmTheta^\T M(\rmX, \rmW),
\end{align}
which is SDGNN with MLP as $h(\cdot)$.

{\bf Completeness of the Function Space of SDGNN.} Regardless of sparsity, we need to show that for $\forall k, \{\rmW_1, \rmW_2, \ldots, \rmW_k\}$, $\rmA$ and $\epsilon>0$, there exists some $\rmTheta$ and $\rmW$, such that when $\rmX$ is within an compact set, we have 
\begin{align}
    \text{sup}_\rmX \|f(\rmX) - g_k(\rmX)\|_F^2 < \epsilon. 
\end{align}

==> sections/arxiv/experiment_log.tex <==
%!TEX root = /Users/yaochen/Dropbox/Apps/Overleaf/yhu-GNN_Efficient_Inference/main.tex
\newpage
\section{Empirical verification on the scale of unique neighbors}
Empirically show the scale of receptive field for each node in different graphs. Uniformly sample 100 nodes and include all the neighbors. Count the non-overlapped number of nodes in this K-hop sub-graph. 

\begin{table}[h]
\caption{Empirical study on the scale of receptive nodes wAnd directly measure the quality of the algorithm by measuring the distance between the original and the approximated neighbor aggregation for each node.ith different layers. $K$ denotes the number of hops.}
\begin{tabular}{llllllll}
\hline
Data          & Features & Nodes   & Edges    & Degrees & $K=1$ & $K=2$   & $K=3$    \\ \hline
Cora          & 1433     & 2708    & 5278     & 3.9     & 4.2   & 36.5    & 128.7    \\
Pubmed        & 500      & 19717   & 44325.5  & 4.5     & 4.5   & 56.4    & 349.2    \\
Reddit        & 602      & 232965  & 57307946 & 492     & 509.7 & 46950.5 & 209951.1 \\
OGBN-arxiv    & 128      & 169343  & 1166243  & 14.8     & 14.8   & 218.3    & 3224.6    \\
OGBN-products & 100      & 2449029 & 61859140 & 50.5    & 50.5  & 2552.0  & 128919.9 \\ \hline
\end{tabular}
\label{tab:nei_size}
\end{table}

Table~\ref{tab:nei_size} shows that unique number of receptive nodes grows even faster than $d^K$, $d$ being the average degree. In fact, the nodes with higher degree are more likely to be hit by other nodes, resulting in a fast expansion of neighbors as number of hop grows. 

\section{How Sampling of Neighbors Influence the GNN Results}
The model is graphSAGE. The model and training configuration is shown in Table~\ref{tab:base_hyper_param}.
\begin{table}[h]
\caption{Training hyper parameters.}
\begin{tabular}{lllll}
\hline
Data          & lr    & hidden size & train sampling size & test sampling size        \\\hline
Cora          & 0.01  & 64 64     & 10                  & 1, 2, 5, 10, 15, 20, full   \\
Pubmed        & 0.01  & 64 64     & 10                  & 1, 2, 5, 10, 15, 20, full   \\
Reddit        & 0.001  & 256 256     & 10               & 1, 2, 5, 10, 15, 20, full \\
OGBN-products & 0.001 & 256 256   & 10                  & 1, 2, 5, 10, 15, 20, full\\\hline
\end{tabular}
\label{tab:base_hyper_param}
\end{table}

All scenarios are run 5 times. The results are shown in Table~\ref{tab:sample_size_impact}. 

\begin{table}[h]
\caption{The impact of sampling size for inference. }
\scalebox{0.7}{
\begin{tabular}{llllllll}
\hline
Data          & 1                 & 2                 & 5                 & 10                & 15               & 20                 & full              \\ \hline
Cora          & $0.7622\pm0.0066$ & $0.7946\pm0.0076$ & $0.8062\pm0.0058$ & $0.8058\pm0.0056$ & $0.8056\pm0.0062$ & $0.8058\pm0.0067$ & $0.8060\pm0.0063$ \\
Pubmed        & $0.7542\pm0.0106$ & $0.7670\pm0.0046$ & $0.7642\pm0.0062$ & $0.7672\pm0.0074$ & $0.7652\pm0.0059$ & $0.7662\pm0.0070$ & $0.7674\pm0.0067$ \\
Reddit        & $0.8067\pm0.0021$ & $0.9247\pm0.0005$ & $0.9554\pm0.0004$ & $0.9606\pm0.0006$ & $0.9619\pm0.0003$ & $0.9627\pm0.0006$ & $0.9640\pm0.0004$ \\
OGBN-products & $0.6802\pm0.0036$ & $0.7509\pm0.0030$ & $0.7769\pm0.0029$ & $0.7819\pm0.0030$ & $0.7832\pm0.0030$ & $0.7836\pm0.0030$ & $0.7844\pm0.0030$
 \\ \hline
\end{tabular}
}
\label{tab:sample_size_impact}
\end{table}

\section{What is the Real Bottleneck of GNN Model Inference}

\subsection{Public Data Sets}
We mainly count two part of time for batch size 1, namely, the time cost to prepare the data including neighbor sampling and the time to actually compute the results via GPU. Statistics are for a random 100 samples. Results are in Table~\ref{tab:time_vs_sampling_size}.
\begin{table}[h]
\caption{Time profiling (second) (sample time / infer time)}
\hspace{-5mm}
\scalebox{0.65}{
\begin{tabular}{l|lllllllll}
\hline
& Neighbor size & 1 & 5 & 20 & 50 & 100 & 200 & full & MLP \\ \hline
\multirow{5}{*}{Reddit} & mean & 0.004/0.005 & 0.004/0.004 & 0.009/0.010 & 0.047/0.025 & 0.130/0.047 & 0.297/0.083 & 3.608/0.312 & 0.00004/0.00035 \\
& 90-percentile & 0.005/0.005 & 0.006/0.005 & 0.011/0.012 & 0.069/0.034 & 0.178/0.066 & 0.457/0.114 & 6.527/0.451 & 0.00005/0.00038 \\
& 99-percentile & 0.007/0.007 & 0.007/0.005 & 0.013/0.014 & 0.079/0.037 & 0.223/0.078 & 0.576/0.133 & 7.581/0.537 & 0.00007/0.00049 \\
& max & 0.008/0.122 & 0.011/0.006 & 0.013/0.015 & 0.081/0.040 & 0.239/0.083 & 0.592/0.135 & 8.741/0.541 & 0.00007/0.00095 \\
& std & 0.001/0.012 & 0.001/0.001 & 0.002/0.002 & 0.018/0.007 & 0.046/0.015 & 0.129/0.026 & 1.937/0.109 & 0.00001/0.00007 \\ \hline

& Neighbor size & 1 & 5 & 20 & 50 & 100 & 200 & full & MLP \\ \hline
\multirow{5}{*}{ogbn-products}& mean & 0.005/0.004 & 0.005/0.004 & 0.006/0.006 & 0.010/0.009 & 0.018/0.010 & 0.034/0.016 & 0.068/0.021 & 0.00004/0.00035 \\
& 90-percentile & 0.005/0.004 & 0.005/0.004 & 0.007/0.008 & 0.015/0.013 & 0.030/0.015 & 0.069/0.025 & 0.147/0.040 & 0.00005/0.00041 \\
& 99-percentile & 0.005/0.005 & 0.007/0.005 & 0.009/0.011 & 0.019/0.015 & 0.042/0.018 & 0.090/0.033 & 0.267/0.051 & 0.00009/0.00073 \\
& max & 0.005/0.005 & 0.007/0.005 & 0.013/0.013 & 0.019/0.016 & 0.053/0.019 & 0.098/0.033 & 0.336/0.054 & 0.00011/0.00074 \\
& std & 0.000/0.000 & 0.000/0.000 & 0.001/0.002 & 0.003/0.003 & 0.009/0.004 & 0.022/0.006 & 0.063/0.012 & 0.00001/0.00010 \\ \hline
\end{tabular}}
\label{tab:time_vs_sampling_size}
\end{table}

\subsection{Internal Data Set}
Data Statistics

\begin{enumerate}
    \item user 1410978
    \item Item 87710
    \item Total edges  18542231
    \item User degree  13.1
    \item Item degree  211.4
\end{enumerate}

Model is 2 layer normal graphSAGE. All 

\begin{enumerate}
    \item sample size, sample time, infer time
    \item 5, 0.0018, 0.0036
    \item 10, 0.0020, na
    \item 15, 0.0036, na
    \item 50, 0.0063, na
\end{enumerate}

\section{A First Exploration of Dictionary Learning Approach}
\subsection{Preliminary Test for Dictionary Learning Based Approximation for Neighbor Information Aggregation}
% We look into the metrics of \emph{regret (R)}
% \begin{align}
%     \text{R} \triangleq \sum_{z\in\gV} \|{\vtheta_z^\T}^\intercal\rmO\rmH - \rmOmega_{z*}\|_2^2,
% \end{align}
% and the \emph{normalized regret (NR)}
% \begin{align}
%     \text{NR} \triangleq \frac{1}{|\gV|}\sum_{z\in\gV} \frac{\|{\vtheta_z^\T}^\intercal\rmO\rmH - \rmOmega_{z*}\|_2^2}{\|\rmOmega_{z*}\|_2^2}.
% \end{align}


% \subsection{How good the dictionary learning can be}
% The main purpose of this experiments is to search through the hyper-parameter space and see the general trend for different data set in order to get a rough idea on the property of the dictionary learning algorithms. 
% \yhc{2022-Dec-2: Due to an implementation bug, the former version approximate the propagation of matrix of with 4 hops, I thought it was 3. }

% The results for Cora dataset are in Table~\ref{tab:dict_cora}.
% \begin{table}[t]
% \caption{Dictionary learning performance for cora dataset. ``a nonzeros'' stands for the number of nonzero entry for the index $\va_z$. ``$\rmO$ resample'' shows how we resample the unused rows of $\rmO$. $WR$, $NWR$, $R$, $NR$ are weighted regret, normalized weighted regret, regret, normalized regret respectively. }
% % \hspace{-5mm}
% \scalebox{1}{
% \begin{tabular}{llllllllll}
% \hline
% Dict size & a nonzeros & $\rmO$ resample & WR & NWR & R & NR & Epoch & Batch size & Time(s)\\\hline
% 50 & 27.1$\pm$5.5 & greedy & 12.150 & 0.319 & 221.838 & 0.869 & 5 & 64 & 99.2\\
% 100 & 20.4$\pm$6.0 & greedy & 8.903 & 0.257 & 186.530 & 0.780 & 5 & 64 & 302.6\\
% 200 & 19.6$\pm$6.5 & greedy & 5.011 & 0.186 & 117.006 & 0.640 & 5 & 64 & 226.5\\
% 400 & 17.6$\pm$6.4 & greedy & 1.791 & 0.095 & 39.732 & 0.380 & 5 & 64 & 426.3\\
% 800 & 15.3$\pm$5.5 & greedy & 0.477 & 0.031 & 10.232 & 0.151 & 5 & 64 & 1315.8\\
% 1600 & 14.2$\pm$5.3 & greedy & 0.084 & 0.005 & 1.492 & 0.028 & 5 & 64 & 3255.8\\\hline
% 50 & 10.3$\pm$3.2 & greedy & 13.200 & 0.346 & 221.547 & 0.860 & 5 & 64 & 83.1\\
% 100 & 10.2$\pm$3.5 & greedy & 9.457 & 0.276 & 184.439 & 0.766 & 5 & 64 & 330.9\\
% 200 & 10.1$\pm$3.7 & greedy & 5.555 & 0.200 & 119.008 & 0.615 & 5 & 64 & 226.2\\
% 400 & 9.2$\pm$3.8 & greedy & 2.131 & 0.111 & 41.946 & 0.389 & 5 & 64 & 582.5\\
% 800 & 8.7$\pm$3.6 & greedy & 0.616 & 0.037 & 11.088 & 0.155 & 5 & 64 & 1425.5\\
% 1600 & 8.7$\pm$4.2 & greedy & 0.139 & 0.008 & 2.106 & 0.031 & 5 & 64 & 4066.3\\\hline
% 50 & 10.4$\pm$3.2 & no & 13.122 & 0.342 & 221.566 & 0.856 & 5 & 64 & 81.6\\
% 100 & 10.1$\pm$3.4 & no & 9.421 & 0.273 & 185.569 & 0.760 & 5 & 64 & 358.2\\
% 200 & 10.1$\pm$3.7 & no & 5.797 & 0.205 & 122.190 & 0.623 & 5 & 64 & 213.4\\
% 400 & 9.4$\pm$3.7 & no & 2.746 & 0.132 & 54.958 & 0.446 & 5 & 64 & 453.8\\
% 800 & 8.8$\pm$3.7 & no & 1.567 & 0.087 & 30.296 & 0.318 & 5 & 64 & 1405.7\\
% 1600 & 8.6$\pm$3.5 & no & 1.055 & 0.062 & 20.495 & 0.237 & 5 & 64 & 3409.1\\\hline
% \end{tabular}
% }
% \label{tab:dict_cora}
% \end{table}

% The results for pubmed dataset are shown in Table~\ref{tab:dict_pubmed}.
% \begin{table}[t]
% \caption{Dictionary learning performance for pubmed dataset. ``a nonzeros'' stands for the number of nonzero entry for the index $\va_z$. ``$\rmO$ resample'' shows how we resample the unused rows of $\rmO$. $WR$, $NWR$, $R$, $NR$ are weighted regret, normalized weighted regret, regret, normalized regret respectively.}
% % \hspace{-5mm}
% \scalebox{1}{
% \begin{tabular}{llllllllll}
% \hline
% Dict size & a nonzeros & $\rmO$ resample & WR & NWR & R & NR & Epoch & Batch size & Time(s)\\\hline
% 200 & 28.6$\pm$6.9 & greedy & 11.456 & 0.096 & 499.325 & 0.844 & 3 & 512 & 3132.9\\
% 500 & 29.0$\pm$8.2 & greedy & 6.922 & 0.064 & 404.661 & 0.738 & 3 & 512 & 10188.5\\
% 1000 & 29.7$\pm$9.7 & greedy & 4.359 & 0.044 & 278.261 & 0.587 & 3 & 512 & 19332.8\\
% 2000 & 29.3$\pm$10.5 & greedy & 2.023 & 0.023 & 129.337 & 0.388 & 3 & 512 & 38609.4\\\hline
% \end{tabular}
% }
% \label{tab:dict_pubmed}
% \end{table}

% \section{Performance of Dictionary Learning Approach on the Specific GCN Tasks}

\subsection{Baselines}
Before we go into the dictionary learning based approaches, we test and compare several important baselines: GraphSAGE model, simple MLP model and fine tuned simplified graph neural network model. Specifically, the fine tuned simplified graph neural network model is the reference upper bound of our approach. As suggested by SGC model, both the MLPs and SGCs adopt row normalization for features. After that, SGC does 2 layer propagation of the features over the symmetric normalized adjacent matrix with self loop added. Ohter parameters are in Table~\ref{tab:base_hyper_param}. The results are shown in Table~\ref{tab:baselines}.
\begin{table}[t]
\caption{Baseline results. ($0/1/2$ means number of hidden layers.)}
% \hspace{-15mm}
\scalebox{0.95}{
\begin{tabular}{lllll}
\hline
Data     & GraphSAGE       & MLP  0/1/2                                          & SGC 0/1/2                                             \\ \hline
Cora     & $0.806\pm0.006$ & $0.597\pm0.001$ / $0.583\pm0.007$ / $0.536\pm0.012$ & $0.800\pm0.004$ / $0.798\pm0.011$ / $0.786\pm0.009$                       \\
Pubmed   & $0.767\pm0.007$ & $0.732\pm0.001$ / $0.717\pm0.017$ / $0.721\pm0.004$ & $0.781\pm0.011$ /  $0.756\pm0.007$ / $0.766\pm0.006$                      \\
Reddit   & $0.964\pm0.000$ & $0.157\pm0.003$ / $0.503\pm0.002$ / $0.626\pm0.003$ & $0.912\pm0.001$ / $0.935\pm0.000$ / $0.937\pm0.000$                       \\
Products & $0.784\pm0.003$ & $0.266\pm0.000$ / $0.418\pm0.001$ / $0.526\pm0.003$ & $0.297\pm0.002$ / $0.489\pm0.002$ / $0.527\pm0.002$                       \\ 
\hline
\end{tabular}
}
\label{tab:baselines}
\end{table}

% \subsection{GCN Performance on Dictionary based Representation}
% Similar to the SGC model, we test the predictive performance over the dictionary based neighbor aggregation and see how it performs. We applied the learned dictionary from the first section of Table~\ref{tab:dict_cora}. The results are shown in Table~\ref{tab:cora_dict_GNN} and Table~\ref{tab:pubmed_dict_GNN}. 

% \begin{enumerate}
%     \item The performance is amazingly good and it is even better than graphSAGE in some setting. The reason might be that the weighted dictionary learning suppressed the noise of the graph and extracted the correlation of nodes from the node features.
%     \item The performance does not necessarily increase as the NWR improves.
% \end{enumerate}

% \begin{table}[t]
% \centering
% \caption{Performance of dictionary learning based GNN for Cora dataset. Learning rates are selected as the same setting with SGC, which is decided by picking the one with best validation accuracy.}
% % \hspace{-15mm}
% \scalebox{0.95}{
% \begin{tabular}{llllll}
% \hline
% Dict size & a nonzeros & NWR & Layer & lr & Accuracy\\\hline
% 50 & 27.1$\pm$5.5 & 0.319 & 0 & 0.5 & 0.823$\pm$0.004\\
% 50 & 27.1$\pm$5.5 & 0.319 & 1 & 0.1 & 0.804$\pm$0.004\\
% 50 & 27.1$\pm$5.5 & 0.319 & 2 & 0.05 & 0.795$\pm$0.013\\
% 100 & 20.4$\pm$6.0 & 0.257 & 0 & 0.5 & 0.822$\pm$0.003\\
% 100 & 20.4$\pm$6.0 & 0.257 & 1 & 0.1 & 0.812$\pm$0.008\\
% 100 & 20.4$\pm$6.0 & 0.257 & 2 & 0.05 & 0.806$\pm$0.012\\
% 200 & 19.6$\pm$6.5 & 0.186 & 0 & 0.5 & 0.811$\pm$0.003\\
% 200 & 19.6$\pm$6.5 & 0.186 & 1 & 0.1 & 0.812$\pm$0.009\\
% 200 & 19.6$\pm$6.5 & 0.186 & 2 & 0.05 & 0.799$\pm$0.009\\
% 400 & 17.6$\pm$6.4 & 0.095 & 0 & 0.5 & 0.808$\pm$0.002\\
% 400 & 17.6$\pm$6.4 & 0.095 & 1 & 0.1 & 0.811$\pm$0.010\\
% 400 & 17.6$\pm$6.4 & 0.095 & 2 & 0.05 & 0.797$\pm$0.013\\
% 800 & 15.3$\pm$5.5 & 0.031 & 0 & 0.5 & 0.794$\pm$0.003\\
% 800 & 15.3$\pm$5.5 & 0.031 & 1 & 0.1 & 0.805$\pm$0.012\\
% 800 & 15.3$\pm$5.5 & 0.031 & 2 & 0.05 & 0.794$\pm$0.013\\
% 1600 & 14.2$\pm$5.3 & 0.005 & 0 & 0.5 & 0.801$\pm$0.002\\
% 1600 & 14.2$\pm$5.3 & 0.005 & 1 & 0.1 & 0.806$\pm$0.013\\
% 1600 & 14.2$\pm$5.3 & 0.005 & 2 & 0.05 & 0.781$\pm$0.006\\ 
% \hline
% \end{tabular}
% }
% \label{tab:cora_dict_GNN}
% \end{table}

% \begin{table}[t]
% \centering
% \caption{Performance of dictionary learning based GNN for Pubmed dataset. Learning rates are selected as the same setting with SGC, which is decided by picking the one with best validation accuracy.}
% % \hspace{-15mm}
% \scalebox{0.95}{
% \begin{tabular}{llllll}
% \hline
% Dict size & a nonzeros & NWR & Layer & lr & Accuracy\\\hline
% 200 & 28.6$\pm$6.9 & 0.096 & 0 & 1 & 0.780$\pm$0.006\\
% 200 & 28.6$\pm$6.9 & 0.096 & 1 & 0.01 & 0.778$\pm$0.003\\
% 200 & 28.6$\pm$6.9 & 0.096 & 2 & 0.1 & 0.776$\pm$0.006\\
% 500 & 29.0$\pm$8.2 & 0.064 & 0 & 1 & 0.777$\pm$0.002\\
% 500 & 29.0$\pm$8.2 & 0.064 & 1 & 0.01 & 0.777$\pm$0.005\\
% 500 & 29.0$\pm$8.2 & 0.064 & 2 & 0.1 & 0.773$\pm$0.004\\
% 1000 & 29.7$\pm$9.7 & 0.044 & 0 & 1 & 0.785$\pm$0.006\\
% 1000 & 29.7$\pm$9.7 & 0.044 & 1 & 0.01 & 0.784$\pm$0.001\\
% 1000 & 29.7$\pm$9.7 & 0.044 & 2 & 0.1 & 0.775$\pm$0.008\\
% 2000 & 29.3$\pm$10.5 & 0.023 & 0 & 1 & 0.789$\pm$0.004\\
% 2000 & 29.3$\pm$10.5 & 0.023 & 1 & 0.01 & 0.786$\pm$0.001\\
% 2000 & 29.3$\pm$10.5 & 0.023 & 2 & 0.1 & 0.777$\pm$0.008\\ 
% \hline
% \end{tabular}
% }
% \label{tab:pubmed_dict_GNN}
% \end{table}

% \begin{table}[t]
% \caption{Dictionary learning performance for Reddit dataset. ``a nonzeros'' stands for the number of nonzero entry for the index $\va_z$. ``$\rmO$ resample'' shows how we resample the unused rows of $\rmO$. $WR$, $NWR$, $R$, $NR$ are weighted regret, normalized weighted regret, regret, normalized regret respectively.}
% % \hspace{-5mm}
% \scalebox{1}{
% \begin{tabular}{llllllllll}
% \hline
% Dict size & a nonzeros & $\rmO$ resample & WR & NWR & R & NR & Epoch & Batch size & Time(s)\\\hline
% 2000 & 74$\pm$7 & greedy & 3395.43 & 0.040 & 98.2 & 0.533 & 2 & 1024 & 61392 \\\hline
% \end{tabular}
% }
% \label{tab:dict_pubmed}
% \end{table}

% \begin{table}[t]
% \centering
% \caption{Performance of dictionary learning based GNN for Reddit dataset. Learning rates are selected as the same setting with SGC, which is decided by picking the one with best validation accuracy.}
% % \hspace{-15mm}
% \scalebox{0.95}{
% \begin{tabular}{llllll}
% \hline
% Dict size & a nonzeros & NWR & Layer & lr & Accuracy\\\hline
% 2000 & 74$\pm$7 & 0.040 & 1 & 0.001 & 0.916$\pm$0.000\\
% 2000 & 74$\pm$7 & 0.040 & 2 & 0.001 & 0.921$\pm$0.000\\
% \hline
% \end{tabular}
% }
% \label{tab:reddit_dict_GNN}
% \end{table}

\section{Complete Tests on Cora}

\subsection{Baseline Results}
{\bf Purposes:} A complete references to the baselines w.r.t time, performance etc.
{\bf Data setting:} The semi-supervised learning way in the work \cite{kipfsemi}. Train/val/test is 140/500/1000.

The baseline results are in Table~\ref{tab:cora_baseline_extended}.

\begin{table}[h]
\caption{The complete baseline tests for Cora}
\label{tab:cora_baseline_extended}
\begin{tabular}{lllll}
\hline
Approach  & \begin{tabular}[c]{@{}c@{}}GNN \\ Layer\end{tabular} & test f1\_mic       & \begin{tabular}[c]{@{}c@{}}Inference time per node \\ (sample/infer) (s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Preprocessing \\ time (s)\end{tabular} \\\hline
MLP0      & 0           & $0.5086\pm0.0010$ & 0.00004/0.00018                            & -                      \\
MLP1      & 0           & $0.5808\pm0.0168$ & 0.00004/0.00028                            & -                      \\
MLP2      & 0           & $0.5050\pm0.0050$ & 0.00003/0.00016                            & -                      \\\hline
SAGE full & 1           & $0.8078\pm0.0075$ & 0.006/0.004                                & -                      \\
SAGE full & 2           & $0.8130\pm0.0067$ & 0.004/0.004                                & -                      \\
SAGE full & 3           & $0.8068\pm0.0066$ & 0.005/0.004                                & -                      \\\hline
SGC0      & 2           & $0.807\pm0.006$   & 0.00003/0.00015                            & 0.0032                 \\
SGC1      & 2           & $0.793\pm0.007$   & 0.00003/0.00023                            & 0.0033                 \\
SGC2      & 2           & $0.759\pm0.018$   & 0.00003/0.00031                            & 0.0046                 \\\hline
SGC0      & 1           & $0.707\pm0.004$   & 0.00003/0.00014                            & 0.0017                 \\
SGC1      & 1           & $0.704\pm0.009$   & 0.00003/0.00026                            & 0.0016                 \\\hline
SGC0      & 3           & $0.785\pm0.005$   & 0.00003/0.00015                            & 0.0073                 \\
SGC1      & 3           & $0.774\pm0.006$   & 0.00003/0.00024                            & 0.0082                \\\hline
\end{tabular}
\end{table}


% \begin{figure}[t]
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includesvg[width=.8\linewidth]{figures/explore_dict_O/norm_O_l1_norm.svg}
%   \caption{1a}
%   % \label{fig:sfig1}
% \end{subfigure}%
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=.8\linewidth]{image2}
%   \caption{1b}
%   % \label{fig:sfig2}
% \end{subfigure}
% \caption{plots of....}
% \label{fig:fig}
% \end{figure}
\subsection{A Converged Working Solution}
{\bf Purpose: } to iteratively find a working solution so that the model performance based on the SDMP is as good as graphSAGE. 
\subsubsection{Results on May. 18 2023}
Table~\ref{tab:0518} shows the performance of this round. Currently there is a large gap between the general case and the SGC based approach. 
% Table generated by Excel2LaTeX from sheet '0519Compare'
\begin{table}[h]
  \centering
  \caption{May 18 Test on Cora}
    \begin{tabular}{lrrrrl}
    \hline
    \textbf{Name} & \multicolumn{1}{l}{\textbf{Dict Size}} & \begin{tabular}[c]{@{}c@{}}\textbf{Normalized} \\\textbf{Regret}\end{tabular} &       & \multicolumn{1}{l}{\textbf{Performance}} &  \textbf{Remark}\\\hline
    SAGEbase 2 layer &       &       &       & \multicolumn{1}{l}{0.8130 ± 0.0067} &  \\
    MLP 1 layer &       &       &       & \multicolumn{1}{l}{0.5808 ± 0.0168} &  \\
    \multicolumn{1}{p{9.5em}}{SGC 1 layer with 2 layer GNN encoder} &       &       &       & \multicolumn{1}{l}{0.807 ± 0.006} &  \\
    \midrule
    Dict learning for SGC & 200   & 0.186 &       & \multicolumn{1}{l}{0.812±0.009} & SGC target \\
    \midrule
    Dict learning for SAGE & 200   & 0.5622 &       & 0.3 \yhc{due to bug}  & General GNN \\
    \end{tabular}%
  \label{tab:0518}%
\end{table}%

\subsection{Tuning and Debugging June 6}
Why the general case does not work? 
\begin{enumerate}
\item the $\rmO$ optimization implementation is wrong.
\item the transformation $\rmH$ is bad.
\item the algorithm cannot learn effective information. 
\end{enumerate}

\subsubsection{Change to the SGC Setting and Test It}
Try align the setting with SGC and see why does not work. Therefore, we use the SGC target as the target for the test. 

Table~\ref{tab:cora_dict_GNN} presents the performance of dictionary learning for SGC models. 

\begin{table}[t]
\centering
\caption{Performance of dictionary learning based GNN for Cora dataset. Learning rates are selected as the same setting with SGC, which is decided by picking the one with best validation accuracy.}
% \hspace{-15mm}
\scalebox{0.95}{
\begin{tabular}{llllll}
\hline
Dict size & a nonzeros & Normalized Regret & Layer & lr & Accuracy\\\hline
50 & 27.1$\pm$5.5 & 0.319 & 0 & 0.5 & 0.823$\pm$0.004\\
50 & 27.1$\pm$5.5 & 0.319 & 1 & 0.1 & 0.804$\pm$0.004\\
50 & 27.1$\pm$5.5 & 0.319 & 2 & 0.05 & 0.795$\pm$0.013\\
100 & 20.4$\pm$6.0 & 0.257 & 0 & 0.5 & 0.822$\pm$0.003\\
100 & 20.4$\pm$6.0 & 0.257 & 1 & 0.1 & 0.812$\pm$0.008\\
100 & 20.4$\pm$6.0 & 0.257 & 2 & 0.05 & 0.806$\pm$0.012\\
200 & 19.6$\pm$6.5 & 0.186 & 0 & 0.5 & 0.811$\pm$0.003\\
200 & 19.6$\pm$6.5 & 0.186 & 1 & 0.1 & 0.812$\pm$0.009\\
200 & 19.6$\pm$6.5 & 0.186 & 2 & 0.05 & 0.799$\pm$0.009\\
400 & 17.6$\pm$6.4 & 0.095 & 0 & 0.5 & 0.808$\pm$0.002\\
400 & 17.6$\pm$6.4 & 0.095 & 1 & 0.1 & 0.811$\pm$0.010\\
400 & 17.6$\pm$6.4 & 0.095 & 2 & 0.05 & 0.797$\pm$0.013\\
800 & 15.3$\pm$5.5 & 0.031 & 0 & 0.5 & 0.794$\pm$0.003\\
800 & 15.3$\pm$5.5 & 0.031 & 1 & 0.1 & 0.805$\pm$0.012\\
800 & 15.3$\pm$5.5 & 0.031 & 2 & 0.05 & 0.794$\pm$0.013\\
1600 & 14.2$\pm$5.3 & 0.005 & 0 & 0.5 & 0.801$\pm$0.002\\
1600 & 14.2$\pm$5.3 & 0.005 & 1 & 0.1 & 0.806$\pm$0.013\\
1600 & 14.2$\pm$5.3 & 0.005 & 2 & 0.05 & 0.781$\pm$0.006\\ 
\hline
\end{tabular}
}
\label{tab:cora_dict_GNN}
\end{table}

Table~\ref{tab:SGC_target_cora} present the performance of the SDMP that use SGC encoder as the target. A few interesting conclusions:
\begin{enumerate}
    \item {\bf The general approach can approximate SGC encoder much better than SAGE encoder.}
    \item Compare SAGE and SGC target, even when SGC target has a worse normalized regret, the f1 micro on the down stream task could perform better than SAGE. Possible reason might be that the f1 score only related to how well the approximated embedding can differentiate the label. 
    \item Sparsity of $\rmO$ is hard to control and sparser $\rmO$ results in bad performance.
\end{enumerate}
All in all, these results show a promising trend that the general setting can still get good performance. And {\bf the quality of $h(\cdot)$ seems to be critical in terms of generating a good performance. }

\begin{table}[h]
	\centering
	\caption{Cora, General Learning Method, SGC Encoder as Target.}
	\begin{tabular}{lllll}
		\hline
		Dict size & Theta nonzeros & O nonzeros & Normalized Regret & f1\_micro\\\hline
		50 & 24.5$\pm$3.9 & 38.0$\pm$174.0 & 0.689 & 0.704$\pm$0.002\\
		50 & 21.9$\pm$3.9 & 1.8$\pm$2.0 & 0.733 & 0.738$\pm$0.006\\
		200 & 38.0$\pm$7.1 & 2.6$\pm$2.6 & 0.568 & 0.773$\pm$0.012\\
		200 & 25.9$\pm$10.4 & 2162.1$\pm$99.8 & 0.272 & 0.809$\pm$0.010\\
		400 & 24.9$\pm$12.2 & 368.3$\pm$349.5 & 0.189 & 0.812$\pm$0.011\\
		400 & 25.3$\pm$12.1 & 388.8$\pm$330.7 & 0.187 & 0.801$\pm$0.010\\\hline
	\end{tabular}
	\label{tab:SGC_target_cora}
\end{table}

\begin{table}[h]
	\centering
	\caption{Pubmed, General Learning Method, SGC Encoder as Target.}
	\begin{tabular}{lllll}
		\hline
		Dict size & Theta nonzeros & O nonzeros & Normalized Regret & f1\_micro\\\hline
		200 & 9.1$\pm$1.3 & 530.6$\pm$900.9 & 0.216 & 0.766$\pm$0.003\\
		200 & 9.2$\pm$1.2 & 598.1$\pm$1093.6 & 0.218 & 0.763$\pm$0.002\\
		500 & 9.9$\pm$0.5 & 18.3$\pm$12.9 & 0.532 & 0.685$\pm$0.007\\
		500 & 9.0$\pm$1.3 & 306.6$\pm$576.6 & 0.267 & 0.748$\pm$0.006\\
		1000 & 8.5$\pm$1.7 & 5784.0$\pm$7641.7 & 0.219 & 0.742$\pm$0.005\\
		1000 & 8.4$\pm$2.1 & 1469.8$\pm$1614.8 & 0.158 & 0.754$\pm$0.007\\\hline
	\end{tabular}
	\label{tab:SGC_target_pubmed}
\end{table}

\subsubsection{Compare the different Optimization for $\rmO$}
To verify the correctness of the optimization procedure for $\rmO$, we initialize the model and train $\rmTheta$ for $1$ epoch. With the same setting, we train the $\rmO$ alone with different algorithms and see the results. 
\begin{figure}[t]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{figures/explore/cora_proximal_NR_O_training.pdf}
  \caption{Proximal algorithm.}
\end{subfigure}%
\caption{Plots of the training curves for various algorithms on Cora dataset.}
\label{fig:fig}
\end{figure}

\section{Direct Decomposition}
{\bf June. 29} We present the results for cora on graphSAGE base to motivate our further studies. We adopt the graphSAGE model with 3 layers as the target GNN encoder. The training batch size is set to 64. The total number of epochs is 5 (empirically, the model converges at about 3 epochs). The results are shown in Table~\ref{tab:cora_SDMP_SAGE}. ``Theta upper'' is the parameter to decide the maximum number of nonzeros in the LAR solver. ``Candidate mode'' shows whether using a candidate set to speed up the training, where ``full'' takes all the nodes as the candidate and ``sparse'' only consider ``base k'' hops of neighbours. ``base k'' shows the $\rmTheta_0$ to initialize $h(\cdot; \rmW)$. Also, in the ``sparse'' mode, we take the ``base k'' hop neighbours for each node as the candidate sets. ``Theta nonzeros'' shows the actually count of nonzeros. ``Normalized Regret'' shows the metric defined in \numref{eq:normalized_regret}. ``SDMP time''
shows the total wall clock time in solving the SDMP. ``f1\_micro'' shows the f1 score on the node classification task based on the SDMP node embeddings. 
\begin{table}[h]
	\centering
	\caption{Cora, SAGE with 3 layers, f1 score of 0.804.}
	\begin{tabular}{lllllll}
		\hline
		Theta upper & Candidate mode & base k & Theta nonzeros & Normalized Regret & SDMP time (s) & f1\_micro\\\hline
		5 & full & 3 & 3.5$\pm$1.0 & 0.038 & 758.0 & 0.795$\pm$0.003\\
		20 & full & 3 & 13.5$\pm$2.6 & 0.002 & 1220.1 & 0.807$\pm$0.003\\
		100 & full & 3 & 37.0$\pm$5.7 & 0.001 & 1645.6 & 0.804$\pm$0.004\\
		100 & sparse & 1 & 2.8$\pm$1.6 & 0.008 & 50.4 & 0.796$\pm$0.003\\
		100 & sparse & 2 & 7.5$\pm$4.3 & 0.004 & 125.1 & 0.809$\pm$0.005\\
		100 & sparse & 4 & 16.8$\pm$7.7 & 0.002 & 425.7 & 0.807$\pm$0.009\\\hline
	\end{tabular}
	\label{tab:cora_SDMP_SAGE}
\end{table}

{\bf June 30. } We test the Pubmed data set in the same setting as Cora. The target GNN encoder is 3-layer SAGE model with a f1 score of 0.774. The testing performance is shown in Table~\ref{tab:pubmed_SDMP_SAGE}.

\begin{table}[h]
	\centering
	\caption{Pubmed, SAGE with 2 layers, f1 score of 0.774.}
	\begin{tabular}{lllllll}
		\hline
		Theta upper & Candidate mode & base k & Theta nonzeros & Normalized Regret & SDMP time & f1\_micro\\\hline
		5 & full & 3 & 4.1$\pm$1.0 & 0.002 & 182289.2 & 0.769$\pm$0.007\\
		20 & full & 3 & 13.8$\pm$2.7 & 0.000 & 185663.8 & 0.768$\pm$0.004\\
		100 & full & 3 & 36.1$\pm$7.6 & 0.000 & 226635.0 & 0.771$\pm$0.003\\
		100 & sparse & 1 & 2.5$\pm$2.3 & 0.007 & 216.9 & 0.742$\pm$0.010\\
		100 & sparse & 2 & 9.6$\pm$6.3 & 0.001 & 763.8 & 0.773$\pm$0.006\\
		100 & sparse & 3 & 18.5$\pm$8.4 & 0.001 & 2692.8 & 0.770$\pm$0.002\\\hline
	\end{tabular}
	\label{tab:pubmed_SDMP_SAGE}
\end{table}

{\bf July 25} Reformulated the implementation and added the sampling for $\vtheta$ candidates and the $\vtheta_0$ to initialize the $h(\cdot)$. Present the new results and check whether the new implementation is consistent. Also, we tested on Reddit dataset. The performance of cora is shown in Table~\ref{tab:core_SDMP_SAGE_new}, pubmed is shown in Table~\ref{tab:pubmed_SDMP_SAGE_new}. 

\begin{table}[h]
	\centering
	\caption{Cora, SAGE with 3 layers, f1 score of 0.809}
        \begin{tabular}{llllllllll}
		\hline
		$\vtheta$ cnt bd & $\vtheta$ mode & $\vtheta$ k1 & $\vtheta$ k2 & $h$ mode & $h$ k & $\vtheta$ 0 cnt & n-Regret & SDMP time & f1\_micro\\\hline
		100 & dense & 1 & 4 & dense & 1 & 2.9$\pm$1.8 & 0.009 & 25.5 & 0.773$\pm$0.006\\
		100 & dense & 2 & 4 & dense & 2 & 8.7$\pm$6.9 & 0.005 & 56.3 & 0.806$\pm$0.005\\
		100 & dense & 3 & 4 & dense & 3 & 13.1$\pm$9.0 & 0.003 & 118.0 & 0.804$\pm$0.008\\
		5 & full & 2 & 4 & dense & 3 & 3.6$\pm$1.1 & 0.020 & 327.7 & 0.807$\pm$0.003\\
		20 & full & 2 & 4 & dense & 3 & 13.6$\pm$3.2 & 0.001 & 451.8 & 0.799$\pm$0.010\\
		100 & full & 2 & 4 & dense & 3 & 29.4$\pm$9.7 & 0.001 & 853.5 & 0.803$\pm$0.006\\
		100 & mixed & 1 & 3 & sparse & 3 & 9.1$\pm$5.4 & 0.004 & 55.9 & 0.794$\pm$0.007\\\hline
	\end{tabular}
	\label{tab:cora_SDMP_SAGE_new}
\end{table}

\begin{table}[h]
	\centering
	\caption{Pubmed, SAGE with 2 layers, f1 score of 0.774}
	\begin{tabular}{llllllllll}
		\hline
		$\vtheta$ cnt bd & $\vtheta$ mode & $\vtheta$ k1 & $\vtheta$ k2 & $h$ mode & $h$ k & $\vtheta$ 0 cnt & n-Regret & SDMP time & f1\_micro\\\hline
		100 & dense & 1 & 3 & dense & 1 & 9.6$\pm$5.0 & 0.001 & 801.9 & 0.768$\pm$0.003\\
		100 & dense & 2 & 3 & dense & 2 & 9.6$\pm$6.0 & 0.001 & 722.2 & 0.766$\pm$0.001\\
		100 & dense & 3 & 3 & dense & 3 & 10.4$\pm$5.6 & 0.001 & 839.3 & 0.770$\pm$0.004\\
		100 & mixed & 1 & 3 & sparse & 3 & 8.5$\pm$5.4 & 0.001 & 671.9 & 0.767$\pm$0.003\\\hline
	\end{tabular}
	\label{tab:pubmed_SDMP_SAGE_new}
\end{table}

\begin{table}[h]
	\centering
	\caption{Reddit, SAGE with 2 layers, f1 score of 0.962}
	\begin{tabular}{llllllllll}
		\hline
		$\vtheta$ cnt bd & $\vtheta$ mode & $\vtheta$ k1 & $\vtheta$ k2 & $h$ mode & $h$ k & $\vtheta$ 0 cnt & n-Regret & SDMP time & f1\_micro\\\hline
		40 & mixed & 1 & 3 & sparse & 3 & 24.6$\pm$3.1 & 0.043 & 35534.9 & 0.954$\pm$0.000\\
		40 & mixed & 1 & 3 & sparse & 3 & 24.5$\pm$3.1 & 0.042 & 168635.9 & 0.954$\pm$0.000\\
		100 & mixed & 1 & 3 & sparse & 3 & 54.3$\pm$4.4 & 0.005 & 45217.6 & 0.955$\pm$0.000\\\hline
	\end{tabular}
	\label{tab:reddit_SDMP_SAGE}
\end{table}

\section{Advanced Experiments for Direct Decomposition}
{\bf Aug. 11} inductive training ablation study on pubmed dataset. Varying the proportion of training node and see the performance under the best performed setting. Table~\ref{tab:pubmed_inductive_train} presented the performance. We can see that the inductive train can still achieve good performance. 

\begin{table}[h]
	\centering
	\caption{Pubmed, SAGE with 2 layers, f1 score of 0.774}
	\begin{tabular}{lllllllllll}
		\hline
		ind ratio & $\vtheta$ cnt bd & $\vtheta$ mode & $\vtheta$ k1 & $\vtheta$ k2 & $h$ mode & $h$ k & $\vtheta$ 0 cnt & n-Regret & SDMP time & f1\_micro\\\hline
		0.2 & 100 & dense & 3 & 3 & dense & 3 & 21.2$\pm$10.3 & 0.001 & 2169.9 & 0.765$\pm$0.003\\
		0.4 & 100 & dense & 3 & 3 & dense & 3 & 20.1$\pm$8.6 & 0.000 & 3692.0 & 0.770$\pm$0.005\\
		0.6 & 100 & dense & 3 & 3 & dense & 3 & 21.9$\pm$9.9 & 0.000 & 5836.6 & 0.777$\pm$0.003\\
		0.8 & 100 & dense & 3 & 3 & dense & 3 & 22.2$\pm$10.3 & 0.000 & 6916.6 & 0.765$\pm$0.008\\\hline
	\end{tabular}
	\label{tab:pubmed_inductive_train}
\end{table}

{\bf Aug. 11} Tune and seek for best performance on Reddit. Look into the factors of adding self as candidate for theta, and use no feature norm. Test the impact of the number of nonzeros for Reddit. Table~\ref{tab:reddit_more_test}. 

\begin{table}[h]
	\centering
	\caption{Reddit, SAGE with 2 layers, f1 score of 0.962, More Tests}
	\begin{tabular}{llllllllll}
		\hline
		$\vtheta$ cnt bd & $\vtheta$ mode & $\vtheta$ k1 & $\vtheta$ k2 & $h$ mode & $h$ k & $\vtheta$ 0 cnt & n-Regret & SDMP time & f1\_micro\\\hline
		40 & mixed & 1 & 3 & sparse & 2 & 24.2$\pm$3.0 & 0.049 & 39995.2 & 0.952$\pm$0.001\\
		40 & mixed & 1 & 3 & sparse & 2 & 24.2$\pm$3.0 & 0.049 & 39995.2 & 0.952$\pm$0.000\\
		40 & mixed & 1 & 3 & sparse & 3 & 24.9$\pm$3.0 & 0.046 & 28564.8 & 0.953$\pm$0.000\\
		40 & mixed & 1 & 3 & sparse & 3 & 24.9$\pm$3.0 & 0.046 & 28564.8 & 0.953$\pm$0.000\\
		150 & mixed & 1 & 3 & sparse & 3 & 61.5$\pm$4.4 & 0.002 & 74096.4 & 0.954$\pm$0.000\\
		150 & mixed & 1 & 3 & sparse & 3 & 61.5$\pm$4.4 & 0.002 & 74096.4 & 0.955$\pm$0.000\\
		300 & mixed & 1 & 3 & sparse & 3 & 62.2$\pm$5.7 & 0.003 & 80661.9 & 0.954$\pm$0.000\\
		300 & mixed & 1 & 3 & sparse & 3 & 62.2$\pm$5.7 & 0.003 & 80661.9 & 0.954$\pm$0.000\\\hline
	\end{tabular}
	\label{tab:reddit_more_test}
\end{table}

\section{Why NR is Low, but the f1 Score can be Bad?}
{\bf Try to align the GNN and the MLP over SDMP.} 

\section{Evidence on Partial Test of Products}
To save the time of hyper-parameter tuning, I only use a partial test for ogbn-product dataset since $90\%$ of the dataset is on testing. To support the claim, I trained an MLP based the features from the RevGNN-112, both the full set testing and a testing with only 0.01 testing samples yielded similar ACC about 0.83. 


==> sections/arxiv/sampling.tex <==
%!TEX root = /Users/yaochen/Dropbox/Apps/Overleaf/yhu-GNN_Efficient_Inference/main.tex
\section{Practical Designs to Boost Convergence}
% \label{sec:tricks}
Although the main algorithm in Sec.~\ref{sec:optimization} is conceptually simple, there are still practical challenges to implementing a robust and scalable algorithm. We describe a few critical design choices and approximations in our implementation that help the convergence. 

\subsubsection{Narrowing the Candidate Nodes}
% \label{sec:append_candi_select}
The computation required to solve \numref{eq:problem_phase_Theta_direct} rapidly grows as the size of $\gV$ increases. Specifically, the computational overhead comes from the inference time of $h(\rmX; \rmW)$ and the computation time of the LARS solver. To reduce the required computation, we define a much smaller candidate node set $\sC_z$ for each node $z$ and only consider the candidate nodes to determine $\vtheta_z$. We solve the following problem instead of \numref{eq:problem_phase_Theta_direct}.
\begin{align}
    \underset{\vtheta}{\text{argmin}} &\quad \frac{1}{2}\|{\vtheta}^\T h(\rmX; \rmW) - {\rmOmega_{z*}}\|_2^2 + \lambda_1 \|\vtheta\|_1 \label{eq:problem_phase_Theta_direct_reduced}\\
    \text{s.t.}&\quad  \vtheta_i \ge 0 \quad \forall i\in \sC_z\\
     &\quad \vtheta_i = 0 \quad \forall i\notin \sC_z.
\end{align}
Here \numref{eq:problem_phase_Theta_direct_reduced_constraint_1} and \numref{eq:problem_phase_Theta_direct_reduced_constraint_2} define the reduced candidate set for solving $\theta_z$. Under this setting, we only need to infer $h(\rmX_{z*}; \rmW)$ for node $z$ that appears in the candidate set and the complexity of the LARS solver only depends on the size of the candidate set instead of $|\gV|$. 

We use the knowledge of the graph structure to heuristically determine the candidate set for each node and aim to include the most relevant nodes with a moderate-sized candidate set.  Specifically, we consider either the $K$-hop neighbours or the nodes sampled during a $K$-hop random walk. We also explore a hybrid, where we take the union of all $K_1$-hop neighbours together with nodes visited during a $K_2$-hop random walk for $K_2>K_1$.

\subsubsection{Stochastic Training}
% \subsubsection{Mini-batch Training} 
{\bf Training on a subset of nodes.} To handle extremely large graphs, we take a random subset of nodes $\gV_t\subset \gV$ before the training loop and train $h(\cdot)$ and $\vtheta_z$ where $z\in\gV_t$. After we have an optimized $h(\cdot)$, we compute the optimized $\rmTheta$ for all $\gV$ over the fixed $h(\cdot)$.

{\bf Mini-batch Training.} We perform mini-batch updates to make the algorithm more efficient. Specifically, we randomly pick $\sB\subset\gV_t$ nodes at each iteration and only update the $\vtheta_z$ where $z\in\sB$. As for $\rmW$, we select the same subset $\sB$ of nodes and the corresponding rows of ${\rmTheta}^\T h(\rmX; \rmW) - {\rmOmega}$ to include in the loss term for each mini-batch, i.e., we solve:
\begin{align}
    \underset{\rmW}{\text{argmin}}\quad \frac{1}{2}\sum_{z\in\sB}\|{\vtheta}_z^\T h(\rmX; \rmW) - \rmOmega_{z*}\|_2^2 + \lambda_2 \|\rmW\|_{F}^2. \label{eq:problem_phase_h_minibatch}
\end{align}

\subsubsection{Warming Up the Feature Transformation}
\label{sec:W_init}

Instead of learning $h(\cdot; \rmW)$ and $\rmTheta$ from random initialization, we can use  knowledge of the graph structure to select a better initial value of $h(\cdot; \rmW)$. Specifically, based on the graph, we create an initial guess $\rmTheta_0$. With fixed $\rmTheta^\T = \rmTheta_0^\T$, we update $h(\cdot; \rmW)$ for a few iterations to warm it up.

We set $\rmTheta_0$ to the $k^{th}$-power of the normalized adjacency matrix, i.e., $\tilde{\rmA}^K$, where $\tilde{\rmA}$ is a symmetric normalized $\rmA$, i.e., $\tilde{\rmA}=\rmD^{-1/2}\rmA\rmD^{-1/2}$ and $\rmD$ is the diagonal matrix where $\ermD_{ii}$ represent the degree of node $i$.
The simple feature propagation has been observed to offer effective performance as a GNN encoder \citep{wu2019simplifying,chen2021graph}. However, computing $\tilde{\rmA}^K$ exactly can be very time-consuming for large graphs. Instead, we adopt random walk and importance sampling techniques to generate an approximation \citep{chen2018fastgcn}. 

\subsection{Algorithm}
Taking into account the design strategies outlined above, the overall algorithm is presented in Algorithm~\ref{alg:main}.
\begin{algorithm}[t]
    \caption{Sparse Decomposition of Graph Neural Networks}
    \label{alg:main}
    \begin{algorithmic}[1] % The number tells where the line numbering should start
        \Procedure{SDGNN}{$\rmOmega, \rmA, \rmX$}
        \State Warm up $\rmW$ according to Section~\ref{sec:W_init}.
        \State Compute the candidate sets $\sC_z$ for each node $z\in\gV$ according to Section~\ref{sec:candi_select}.
        \State Randomly pick a subset $\gV_t\subset\gV$ for inductive training. 
        \For{$t=1$ to $T$}\Comment{Main training loop.}
            \State Get the current mini-batch of node set $\sB_t\subset\gV_t$.
            \For{each $z$ in $\sB_t$}
                \State Update $\vtheta_z$ with the solution of the problem in \numref{eq:problem_phase_Theta_direct_reduced} with LAR algorithm.
            \EndFor
            \State Update $\rmW$ with the loss as \numref{eq:problem_phase_h_minibatch} for a few iterations with SGD.
        \EndFor
        \For{each $z$ in $\gV$} \Comment{Fix $\rmW$ and finalize the $\rmTheta$.} \label{alg:line_post_process}
                \State Update $\vtheta_z$ with the solution of the problem in \numref{eq:problem_phase_Theta_direct_reduced} with LAR algorithm.
            \EndFor
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

\section{Random Walks and Importance Sampling on Normalized Adjacent Matrix}
\label{sec:random_walk}
Given a predefined hop $K$, we recursively node-wisely sample the neighbours and determine the weight. Specifically, we have a predefined budget list $\{s_1, s_2, \ldots, s_K\}$, where we sample $s_k$ nodes at layer $k$. Let $p_{ij}$ defines the sampling probability that node $j$ will be included as a neighbour of node $i$, and $\vp_i$ is $|\gV|$ dimension vector $[ p_{i1}, p_{i2}, 
\ldots, p_{i|\gV|}]^\T$. We perform forward sampling and backward aggregation to evaluate the desired sparse approximation matrix $\bar{\rmA}^K$, which approximates $\tilde{\rmA}^K$. At each iteration, we take a mini-batch of nodes $\sB\in\gV$ and compute the rows of $\bar{\rmA}^K$ with the row indices in $\sB$.

{\bf Forward sampling.} At layer $k$, suppose we have a collection of seed nodes $\sS^{(k)}$. For each node $z\in\sS^{(k)}$, we bootstrap sample $s_{k+1}$ nodes according to $\vp_z$ and get a \emph{multiset} collection $\sS^{(k+1)}_z$. Then we produce the seed node set by taking union and unique operation overall $\sS^{(k+1)}_z$, i.e.,
\begin{align}
    \sS^{(k+1)} = \bigcup_{z\in\sS^{(k)}}\text{Set}(\sS^{(k+1)}_z), \label{eq:forward_sampling_set}
\end{align}
where we denote $\text{Set}(\cdot)$ as the operation to convert a multiset into a normal set. 
We set $\sS^{(0)}:=|\sB|$, and recursively generate $\sS^{(k)}_z$, and $\sS^{(k)}$ for $\{(k, z)\mid k=1,2,\ldots,K, z\in\sS^{(k)}\}$. 

Note that the union operation in \numref{eq:forward_sampling_set} helps to reduce overhead of doing repeated sampling for the same nodes, which is akin to the idea of layer-wise sampling \cite{chen2018fastgcn}.

{\bf Backward aggregation.} For $k=1,2,\ldots,K-1$, we define the auxiliary set of sparse representations to conduct efficient computation for the rows of $\bar{\rmA}^K$ within $\sB$ in a dynamic programming manner. Specifically, for some $k\in [1, K]$ and $k\in \sN$, we define \emph{sparse vector} $\sA^{(k)}_z:=\{(i, w(i))\in (\sN^+, \sR)\}$ for $\forall z\in\sS^{k-1}$, where $(i, w(i))$ denotes the index $i$ of nonzero entry and the corresponding weight $w(i)$. Define the sum of two sparse vector $\sA_1$ and $\sA_2$ as $\sA_1+\sA_2:=\{\big(i, w_{\sA_1}(i)+w_{\sA_2}(i)\big)\mid\forall i\in \text{Supp}(\sA_1)\cup\text{Supp}(\sA_2)\}$, where $w_{\sA}(i)$ denotes the $w(i)$ in the sparse vector $\sA$ and $w(i):=0$ if $i\notin \text{Supp}(\sA)$. Define the multiplication between a sparse vector $\sA$ and a scalar $a$ as $\sA a=a\sA:=\{\big(i, a\cdot w_{\sA}(i)\big)\mid\forall i\in \text{Supp}(\sA)\}$.
% Define the element-wise multiplication between a normal vector $\va$ and the sparse vector $\sA$ as $\va\odot\sA=\sA\odot\va:=\{\big(i, w_{\sA}(i)\cdot a_i\big)\mid\forall i\in\text{Supp}(\sA)~\text{and}~a_i\neq 0\}$.
We abuse the equality notation between a \emph{sparse vector} and a normal vector, i.e., we write $\sA=\vv$ or $\vv=\sA$ iff. 
\begin{align}
    v_i = \begin{cases}
                w_{\sA}(i) \quad&\text{if }i\in\text{Supp}(\sA), \\
                0\quad &\text{otherwise}.
          \end{cases}
\end{align}
% Define the eliment-wise inverse of $\vp_z$ as $\vp_z^{-1}$, where 
% \begin{align}
%     p^{-1}_{zi} = \begin{cases}
%                         \frac{1}{p_{zi}} \quad\text{if }p_{zi}\neq 0, \\
%                         0\quad \text{otherwise}.
%                   \end{cases}
% \end{align}
Define $\sA^{(K)}_i:=\{(i, 1)\}$ for $\forall i\in|\gV|$. Recursively, we define 
% \begin{align}
%     \sA^{(k)}_z:=\frac{1}{s_{k+1}}\tilde{\rmA}_{z*}\odot\sum_{i\in\sS^{(k+1)}_z} \frac{1}{p_{zi}}\sA^{(k+1)}_i.
% \end{align}
\begin{align}
    \sA^{(k)}_z:=\frac{1}{s_{k+1}}\sum_{i\in\sS^{(k+1)}_z} \frac{\tilde{\ermA}_{zi}}{p_{zi}}\sA^{(k+1)}_i.
\end{align}
Note that we implicitly add multiple copies of $\sA^{(k+1)}_i$ if $i$ appears multiple times in the multiset $\sS^{(k)}_z$. Finally, the $\sA^{(0)}_z$ for $\forall z\in\sB$ are the sparse representations of rows of $\bar{\rmA}^K$ within $\sB$.

{\bf The unbiased sampling.} For consistency of notation, let us define $\tilde{\rmA}^0:=\rmI$. 
\begin{proposition} \label{prop:unbiased_sampling}
    With predefined $\vp_z$ for $\forall z$, $\tilde{\rmA}$ and $K$, for $\sA^{(k)}_z$, $\forall k,z$ defined in the forward sampling and backward aggregation, we have that the expected sparse vector $\Ex_{\sS^{(k+1)}_z, \{\sS^{(j)}_x \mid \forall j\ge k+2, \forall x\}} \left(\sA^{(k)}_z\right)$ represents exactly ${\tilde{\rmA}^{K-k}}_{z*}$ for $k=0, 1, \ldots, K-1$ and $\forall z\in \sS^{(k-1)}$.
\end{proposition}
\begin{proof}
We prove it by induction on $k$. For $k=K-1$ and $\forall z\in\sS^{(K-1)}$, we have
\begin{align}
    \Ex_{\sS^{(k+1)}_z, \{\sS^{(j)}_x \mid \forall j\ge k+2, \forall x\}} \left(\sA^{(K-1)}_z\right) &= \Ex_{\{\sS^{(K)}_x \mid \forall x\}} \left(\frac{1}{s_{K}}\sum_{i\in\sS^{(K)}_z} \frac{\tilde{\ermA}_{zi}}{p_{zi}}\sA^{(K)}_i \right)\nonumber\\
    &= \frac{1}{s_{K}}\sum_{i\in\sS^{(K)}_z} \Ex_{\sS^{(K)}_z} \left(\frac{\tilde{\ermA}_{zi}}{p_{zi}}\sA^{(K)}_i \right) \nonumber\\
    &=  \Ex_{i\sim \vp_z} \left(\frac{\tilde{\ermA}_{zi}}{p_{zi}}\sA^{(K)}_i \right)\nonumber\\
    &= \sum_{i} \tilde{\ermA}_{zi} \sA^{(K)}_i\nonumber\\
    &= \tilde{\rmA}_{z*}^{K - (K-1)}. \nonumber
\end{align}
Suppose for some $k\in \sN, 1\le k\le K-1$ and $\forall z\in\sS^{k-1}$, we have $\Ex_{\{\sS^{(j)}_x \mid \forall j\ge k+1, \forall x\}} \left(\sA^{(k)}_z\right) = {\tilde{\rmA}^{K-k}}_{z*}$, for $k-1$ we can get
\begin{align}
    \Ex_{\sS^{(k)}_z, \{\sS^{(j)}_x \mid \forall j\ge k+1, \forall x\}} \left(\sA^{(k-1)}_z\right) &= \Ex_{\sS^{(k)}_z, \{\sS^{(j)}_x \mid \forall j\ge k+1, \forall x\}} \left(\frac{1}{s_{k}}\sum_{i\in\sS^{(k)}_z} \frac{\tilde{\ermA}_{zi}}{p_{zi}}\sA^{(k)}_i\right)\nonumber\\
    &=\frac{1}{s_{k}}\sum_{i\in\sS^{(k)}_z} \Ex_{\sS^{(k)}_z, \{\sS^{(j)}_x \mid \forall j\ge k+1, \forall x\}} \left(\frac{\tilde{\ermA}_{zi}}{p_{zi}}\sA^{(k)}_i\right)\nonumber\\
    &=\frac{1}{s_{k}}\sum_{i\in\sS^{(k)}_z} \Ex_{\sS^{(k)}_z} \left(\frac{\tilde{\ermA}_{zi}}{p_{zi}}\Ex_{\{\sS^{(j)}_x \mid \forall j\ge k+1, \forall x\}}\left(\sA^{(k)}_i\right)\right)\nonumber\\
    &=\Ex_{i\sim\vp_z} \left(\frac{\tilde{\ermA}_{zi}}{p_{zi}}\Ex_{\sS^{(k+1)}_i,\{\sS^{(j)}_x \mid \forall j\ge k+2, \forall x\}}\left(\sA^{(k)}_i\right)\right)\nonumber\\
    &=\sum_i \tilde{\ermA}_{zi} \tilde{\rmA}^{K-k}_{i*}\nonumber\\
    &=\tilde{\rmA}^{K-(k-1)}_{z*},\nonumber
\end{align} 
Completing the proof. \hfill\qed
\end{proof}

{\bf Definition of $\vp_z$.} Like \cite{chen2018fastgcn}, we analyze the variance of $\sA^{(k)}_z$ and minimize the variance w.r.t. $\vp_z$. However, the full variance is challenging to compute. Instead, we inspect the variance with the randomness from $\sS^{(k+1)}_z$ and fix the other random variables, i.e., we define
\begin{align}
    \valpha^{(k)}_z := \frac{1}{s_{k+1}}\sum_{i\in\sS^{(k+1)}_z} \frac{\tilde{\ermA}_{zi}}{p_{zi}}\tilde{\rmA}^{K-(k+1)}_{i*},
\end{align}
which can be regarded as a mean of $s_{k+1}$ i.i.d. random variables $\valpha:=\frac{\tilde{\ermA}_{zi}}{p_{zi}}\tilde{\rmA}^{K-(k+1)}_{i*}$ with a probability of $\vp_z$. From the proof of Proposition~\ref{prop:unbiased_sampling}, we can get $\Ex(\valpha^{(k)}_z)=\Ex(\valpha)={\tilde{\rmA}^{K-k}}_{z*}$. Computing the trace of the covariance matrix
\begin{align}
    \text{Var}(\valpha) &= \Ex_{i\sim\vp_z} \left(\left(\frac{\tilde{\ermA}_{zi}}{p_{zi}}\tilde{\rmA}^{K-(k+1)}_{i*} -  {\tilde{\rmA}^{K-k}}_{z*}\right) \left(\frac{\tilde{\ermA}_{zi}}{p_{zi}}\tilde{\rmA}^{K-(k+1)}_{i*} -  {\tilde{\rmA}^{K-k}}_{z*}\right)^\T\right)\nonumber\\
    &= \sum_i \frac{1}{p_{zi}}\tilde{\ermA}_{zi}^2 \|\tilde{\rmA}^{K-(k+1)}_{i*}\|_2^2 - 2\sum_i \tilde{\ermA}_{zi}\langle \tilde{\rmA}^{K-(k+1)}_{i*}, \tilde{\rmA}^{K-k}_{z*}\rangle  + \|\tilde{\rmA}^{K-k}_{z*}\|_2^2\nonumber\\
    &= \sum_i \frac{1}{p_{zi}}\tilde{\ermA}_{zi}^2 \|\tilde{\rmA}^{K-(k+1)}_{i*}\|_2^2 - \|\tilde{\rmA}^{K-k}_{z*}\|_2^2.
\end{align}
Therefore, 
\begin{align}
    \text{Var}(\valpha^{(k)}_z) = \frac{1}{s_{k+1}}\text{Var}(\valpha) 
    = \frac{1}{s_{k+1}}\sum_i \frac{1}{p_{zi}}\tilde{\ermA}_{zi}^2 \|\tilde{\rmA}^{K-(k+1)}_{i*}\|_2^2 - \frac{1}{s_{k+1}}\|\tilde{\rmA}^{K-k}_{z*}\|_2^2.
\end{align}
Let $c_i:=\tilde{\ermA}_{zi}^2\|\tilde{\rmA}^{K-(k+1)}_{i*}\|_2^2 \ge0$ for $\forall i$, we have
\begin{align}
    \sum_i \frac{1}{p_{zi}}c_i &= \sum_i (\sqrt{\frac{c_i}{p_{zi}}})^2 \sum_i (\sqrt{p_{zi}})^2\nonumber\\
    &\ge \left(\sum_i \sqrt{\frac{c_i}{p_{zi}}}\sqrt{p_{zi}}\right)^2
    = \left(\sum_i \sqrt{c_i}\right)^2, 
\end{align}
where the equality holds, i.i.f. $p_{zi}\propto\sqrt{c_i}$ for $\forall i$. Therefore, we should take
\begin{align}
    p_{zi}\propto \tilde{\ermA}_{zi}\|\tilde{\rmA}^{K-(k+1)}_{i*}\|_2,
\end{align}
to minimize the variance. However, $\|\tilde{\rmA}^{K-(k+1)}_{i*}\|_2$ is expensive to compute for all $k$. Empirically, we take $p_{zi}\propto \tilde{\ermA}_{zi}\|\tilde{\rmA}_{i*}\|_2$.

% {\bf Complexity Analysis.} \yhc{add complexity later.}

==> sections/dynamic_task_exp_focus_on_generalization.tex <==
\onecolumn
\section{Dynamic Task: Exploration on SDGNN's Generalizability for Evolving Features}


% \mai{Since it is like a new task and I don't think the problem statement in Sec 4.2 is sufficient to describe this therefore I made a new problem statement and experiment plan here}

To verify SDGNN's generalizability on inference time given evolving node attributes compared to baseline models (e.g., GLNN and NOSMOG),
we conduct the comparison experiments based on T-GCN framework ~\citep{zhao2020tgcntemporalgraph} on spatio-temporal datasets.
To verify the generalizability, 
we replace the original spatial feature encoder (i.e., GCN) in T-GCN with the frozen pre-trained SDGCNN/GLNN/NOSMOG/GCN and train the temporal fracture encoder (i.e., GRU) solely (as shown in Fig.~\ref{fig:overview_tgcn}).

\textbf{Note that the goal is to verify the generalizability of SDGNN instead of showcasing its capacity to capture temporal dependencies.}

% We'll use spatial-temporal datasets, to provide this evolving context. Rather than comparing against SOTA spatial-temporal models, \textbf{our focus is solely on showcasing SDGNN's performance in evolving data scenarios}. Our proposed experiment framework is as follows:




\subsection{Proposal Experiment -- Graph Embedding encoder with RNN decoder}




We aim to utilize the existing SDGNN model, as previously developed by Yaochen, exclusively as an encoder for generating embeddings, pairing it with an RNN to serve as the decoder for temporal downstream tasks. This methodology will be similarly applied to the GLNN and NOSMOG models. Concurrently, we plan to assess the performance of a GCN used in the encoder role for embedding production. The overarching architecture of our model, along with the conceptualization of the downstream task, is influenced by the T-GCN framework as detailed by \cite{zhao2020tgcntemporalgraph}. 

\subsubsection{Downstream problem definition}

The goal of our downstream task is to predict future traffic conditions, such as speed, flow, and density, using historical traffic data on road networks. Following the approach in \cite{zhao2020tgcntemporalgraph}, we focus on traffic speed for our experiments. We model the road network as an unweighted graph $G = (V, E)$, where each road is a node ($V = {v1, v2, ..., vN}$, with $N$ being the total number of nodes) and edges ($E$) represent connections between roads. The adjacency matrix $A$, consisting of 0s and 1s, indicates these connections. The task involves using past feature matrices $X_{t-n}, ..., X_{t-1}$ to predict future traffic information $Y_t$. This task serves to test the SDGNN model's effectiveness in handling evolving traffic features.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/evolving_feature_generalizability_exp/tgcn/overview_tcgn.png}
    \caption{Overview of T-GCN architecture \citep{zhao2020tgcntemporalgraph}. It takes the historical traffic information as input and obtain the finally prediction result through the Graph Convolution Network and the Gated Recurrent Units model. }
    \label{fig:overview_tgcn}
\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/evolving_feature_generalizability_exp/tgcn/detailed_view_tcgn.png}
    \caption{The overall process of spatio-temporal prediction \citep{zhao2020tgcntemporalgraph}. The right part represents the specific architecture of a T-GCN unit, and GC represents graph convolution.}
    \label{fig:detailed_tgcn}
\end{figure}

\subsubsection{Metrics}
\begin{itemize}
    \item RMSE
    \begin{align}
        RMSE = \sqrt{\frac{1}{n}\sum^n_{i=1} (Y_t - \hat{Y}_t)^2}
    \end{align}
    \item MAE
    \begin{align}
        MAE = \frac{1}{n}\sum^n_{i=1}|Y_t - \hat{Y}_t|
    \end{align}
    \item Coefficient of Determination (R2)
    \begin{align}
        R^2 = 1 - \frac{\sum_{i=1} (Y_t - \hat{Y}_t)^2}{\sum_{i=1} (Y_t - \bar{Y})^2}
    \end{align}
\end{itemize}


\subsubsection{T-GCN Architecture}
% We plan to borrow T-GCN architecture to conduct this experiment since we think T-GCN is neat enough to distinguish the effect down by the graph embedding and the 
\label{sec:tgcn}
\begin{align}
    u_t =& \sigma (W_u [f(A, X_t), h_{t-1}] + b_u) \\
    r_t =& \sigma (W_r [f(A, X_t), h_{t-1}] + b_r) \\
    c_t =& tanh(W_c[f(A,X_t), (r_t*h_{t-1}] + b_c) \\
    h_{t} =& u_t * h_{t-1} + (1-u_t) * c_t 
    \label{eq:tgcn_gru}
\end{align}


Equation \ref{sec:tgcn} presents the structure of our foundational model, in which $f(A, X_t)$ denotes the graph convolution process as detailed in \cite{zhao2020tgcntemporalgraph}. \textbf{This process ultimately yields embeddings derived from pre-trained models such as GCN, GLNN, NOSMOG, or SDGNN within our experimental framework.} Here, $X_t$ represents the feature matrix and $A$ the adjacency matrix. The activation function is denoted by $\sigma(\cdot)$. The variables $u_t$ and $r_t$ correspond to the update and reset gates at time $t$, respectively, while $h_t$ signifies the output at that time. Figure \ref{fig:overview_tgcn} illustrates the overall structure of the T-GCN model. Our objective is to explore substitutions of the GCN component with alternatives like GLNN, NOSMOG, or SDGNN. Figure \ref{fig:detailed_tgcn} provides a detailed depiction of the T-GCN model, highlighting the integration of the GRU mechanism.


% Eq.\ref{sec:tgcn} listed the architecture of our based model, where $f(A, X_t)$ are the graph convolution process in \cite{zhao2020tgcntemporalgraph} but it is eventually the embedding extracted from either pre-trained GCN, GLNN, NOSMOG or SDGNN in our experiment setting, $X_t$ is the feature matrix, $A$ is the adjacency matrix. $\sigma(\cdot)$ is the activation function. $u_t$, $r_t$ are update gate and reset gate at time $t$, and $h_t$ denotes the output at time $t$. Fig.\ref{fig:overview_tgcn} shows the overview of the T-GCN architecture as well, what we want to do is to change the \textbf{GCN} to \textbf{GLNN}, \textbf{NOSMOG}, \textbf{SDGNN}. Fig.\ref{fig:detailed_tgcn} shows the detailed view in T-GCN, where shows how the GRU comes into the play.


% Treat trained SDGNN, GLNN/NOSMOG, GCN as an encoder and generate embedding, and use sequence model (like RNN) to do the downstream forecasting task.

we want to show that as for generalizability power, 

\begin{equation*}
    \textbf{GCN} \ge \textbf{SDGNN} > \{\textbf{GLNN}, \textbf{NOSMOG} \}
\end{equation*}
\mai{Or even $\textbf{SDGNN} \ge \textbf{GCN}$, maybe}


\newpage

==> sections/prepare_for_rebuttal.tex <==
\newpage

\section{Train with more epochs}

We found out that with a schedule: With total 8000 training epochs, we gradually reduced the receptive field size. Specifically, every 100 epochs, the maximum receptive field size was decreased by 1. We found that the receptive field for  



\section{3-hop GCN experiment}

Figure \ref{fig:scatter_pem08_3} shows the results with 3 layer GCN. 

\begin{figure}[t]
     \centering
     \includegraphics[width=0.45\textwidth]{figures/scatter_plot_with_error_bars_with_3.pdf}
     \vspace{-1em}
     \caption{MAPE v.s. mean receptive field size on PeMS08 dataset with 3 layer GCN. L1, L2 denote one and two GCN layers, respectively. GLNN and MOSMOG are learned with GRU-GCN-L2. Targets of SDGNN are indicated in brackets. Error bar shows standard deviation.}
     % \vspace{-1em}
    \label{fig:scatter_pem08_3}
\end{figure}


==> sections/rebuttal.tex <==
\section{Reviews}

\subsection{Reviewer M5fg / Reviewer 1}
{\bf Summary Of Contributions:}

The authors introduce SDGNN, an MLP-based method for approximating GNN embeddings that is linear w.r.t. average node degree and the number of layers in the GNN. Subsuming prior work with heuristic decoupling and knowledge distillation, SDGNN is novel in its approach by alternating between training an MLP to approximate the teacher GNN embeddings and optimizing sparse weights. This enables fast inference where each node embedding is computed as a linear combination of the other embeddings using those sparse weights. Through thorough experiments on graph and temporal graph node classification benchmarks, SDGNN outperforms existing methods with superior inference efficiency.

{\bf Strengths And Weaknesses:}

Strengths

Temporal graph benchmarks: MLP-based graph GNN approximators are usually not benchmarked on temporal graph datasets, so it is a pleasant comparison to see how models perform in a different setting than the usual graph

General formulation: SDGNN has the benefit of being more general than what the authors describe as "heuristic decoupling" approaches, and it's clear how its weights can be adjusted to subsume PPR/normalized adjacency matrix methods. This introduces new optimization challenges, which adds to the novelty of the paper.

Comprehensive experiments: Experiments and results are very well-presented, and significance testing is used in the main results. All hyperparameters and optimization schedules are transparently described in detail in the Appendix.

Weaknesses

Missing baselines/benchmarks: The authors are missing comparison with VQGraph [1], a new SOTA GNN-MLP distillation technique. I think comparison with this method would be beneficial. Also, Table 2 only shows results for homophilic graph datasets. Performance on heterophilic datasets with heterophily-minded GNN teachers would be helpful for evaluating SDGNN.

Lack of asymptotic analysis: Especially for training SDGNN, the paper would benefit from an explicit analysis of the time complexity of SDGNN taking into account both the candidate node generation algorithm and the LARS solver.

Lack of ablation/sensitivity studies: There are several hyperparameters that are important for SDGNN's performance, such as 
, 
, the number of LARS iterations, 
, and 
. It would be helpful to know how SDGNN performs differently w.r.t. different settings of these parameters.
Lack of training time cost SDGNN requires both training a neural network with gradient descent and solving an optimization problem with a LARS solver. It seems SDGNN's training procedure can be quite expensive, requiring training for 4000 epochs alternating between training the MLP and the sparse weights. A discussion on the time and space costs of training SDGNN complete with a study examining how each component affects training/inference time would be helpful. As it stands, it seems SDGNN should be no cheaper to train than models like SAGE with few layers and small neighborhood size < .

[1] VQGraph: Rethinking Graph Representation Space for Bridging GNNs and MLPs

Requested Changes:

Can the authors elaborate on a more intuitive explanation for what SDGNN boils down to on an intuitive way? It seems SDGNN is essentially a way of conducting weighted message passing with teacher GNN supervision and sparse edge weights, but a clear intuition behind the method would be helpful given the difficult interpretability of sparse weights.

Can the authors elaborate on the importance of each component of SDGNN on downstream performance/inference time? For instance, in Appendix D.4, the authors note that different strategies in optimizing the sparse weights can result in tradeoffs between computation complexity and accuracy. Further, how much do hyperparameters such as max LARS iterations and 
 and 
 affect performance?
 
Can the authors elaborate on what the significance of dynamic node features with the shortcomings of existing GNN/MLP models in fast dynamic node inference? This advantage is mentioned in the beginning sections, but the explicit connection between dynamic node features and the temporal graph benchmark as well as explaining why SDGNN is superior in this regard could use more detail.
Broader Impact Concerns:
N/A

Claims And Evidence: Yes
Audience: Yes

\subsection{Reviewer bvcp / Reviewer 2}
Summary Of Contributions:
The paper introduces SDGNN, a novel method for efficiently approximating GNN node representations. The key innovation is combining learned feature transformations with sparse weight vectors to determine which transformed node features to aggregate, allowing efficient approximation of GNN embeddings.

Unlike prior MLP-based approximations, SDGNN can process neighbor features during inference while maintaining linear complexity. It provides a principled way to trade off between approximation quality and inference efficiency through sparsity constraints, though with some limitations in inductive settings and non-linear feature interactions.

Strengths And Weaknesses:
Strengths

The work addresses an important practical problem of making GNN inference more efficient for online prediction while preserving model quality. The solution is well-motivated and technically sound.
The empirical validation is thorough and convincing, with extensive experiments across different datasets, model architectures, and application settings (node classification and spatio-temporal forecasting).
The method is flexible and can approximate various GNN architectures while maintaining linear complexity. The authors demonstrate this by successfully applying SDGNN to GraphSAGE, Geom-GCN, Exphormer and other architectures.
The authors provide clear comparisons with existing approaches and demonstrate meaningful improvements over state-of-the-art methods.
Weaknesses

The theoretical analysis is limited. The paper would benefit from formal analysis of SDGNN's expressiveness compared to standard GNNs and theoretical guarantees on approximation quality. I'm particularly interested in why the GNN's performances are improved after the decomposition. Is it possible to add some (heuristic) explanations? Such as visualise these embeddings?
The approach has limited ability to capture non-linear interactions between node features, which may be important for some applications. This fundamental limitation deserves more discussion.
The method cannot handle inductive settings where new nodes appear during inference. While the authors acknowledge this limitation, more discussion of potential solutions would be valuable.

Requested Changes:

Requested Changes

Include a theoretical/empirical analysis section examining SDGNN's expressiveness compared to standard GNNs. At minimum, identify conditions under which SDGNN can/cannot match/imporve GNN performance.

Suggested Improvements

Add experiments showing how performance degrades with increasing time gaps between training and testing in the spatio-temporal setting.

Include an analysis of memory requirements alongside the existing computational complexity discussion.

Provide a detailed discussion of strategies for handling distribution shift in online/streaming settings. This is essential since the method is aimed at online prediction scenarios where data distributions may evolve over time.

Add experiments on more diverse types of graph data beyond citation networks and traffic forecasting.

Provide guidelines for selecting key hyperparameters like K1 and K2 based on graph properties.

Broader Impact Concerns:
NO

Claims And Evidence: Yes
Audience: Yes

\subsection{Reviewer Vd3Z / Reviewer 3}
Summary Of Contributions:

The paper presents an approach called SDGNN that reduces inference time by approximating node representations through a weighted sum of features from a carefully selected subset of nodes, achieving linear complexity with respect to the average node degree and the number of layers.

Strengths And Weaknesses:

Strengths:

The paper is well-structured and easy to follow, with clear explanations of the proposed method and its components.

The experimental results are comprehensive, demonstrating the effectiveness of SDGNN across various datasets and tasks.

The approach is innovative in its use of sparse decomposition to maintain model accuracy while significantly reducing inference time.

Weaknesses:

How does the method handle the introduction of new nodes in an inductive learning setting, given that it requires pre-computed embeddings for all nodes?

Is there a risk of losing important non-linear interactions between node features due to the linear combination used in the sparse decomposition?

How does the training time and computational complexity scale with very large graphs?

How does the method ensure that the sparse weight vectors $\theta z$ remain non-negative during the optimization process, as indicated by the constraint in equation (5)?

In the context of narrowing the candidate nodes, how does the heuristic approach for selecting the candidate set impact the model's ability to capture important node features?

Requested Changes:

See Weaknesses

Broader Impact Concerns:
NA

Claims And Evidence: Yes
Audience: Yes

\section{Summary of Issues}

\subsection{Reviewer M5fg / Reviewer 1}
\begin{enumerate}
    \item {\bf Discuss VQGraph paper}
    \item Heterophilic dataset
    \item Training complexity analysis.
    \item Sensitivity analysis of K1 and K2, lambda 1 and lambda 2.
    \item Training time analysis. Component to demonstrate the training time.
    \item
    \item Explain the intuition of the method and how this is different from a weighted message passing. Intuition: why does this work? Perhaps theory on the expressiveness?
    \item Analyse how the hyper-parameters influence the performance and time?
    \item Elaborate with the change of different settings of parameters
    \item Explain the significance of dynamic node features. How SDGNN is better than GNN/MLP models. 
\end{enumerate}

\subsection{Reviewer bvcp / Reviewer 2}
\begin{enumerate}
    \item Theoretical analysis of expressiveness of SDGNN.
    \item Why the performance could be better than GNN. Visualize the embeddings?
    \item more discussion on limitation for non-linear interaction. 
    \item \st{issue for inductive setting. need to provide a potential solution.}
    \item 
    \item theoretical or empirical analysis on the expressiveness of SDGNN. 
    \item Add experiments showing how performance degrades with increasing time gaps. \yhc{TODO Mai}
    
    \item Add memory requirement.
    \item \st{strategy for distribution shit.}
    \item Add experiments on more diverse types of graph data beyond citation and traffic forecasting.
    \item Guidelines for parameters selection like $K_1$ and $K_2$ based on graph properties. 
\end{enumerate}

\begin{itemize}
    \item In this experiment, we analyze the prediction error between the ground truth and predicted values by calculating the absolute error for each data point. The absolute error list is then divided into 10 equal-sized chunks, preserving the chronological order of the data. Shown in Figure \ref{fig:mae_distribution_shift}, for each chunk, the mean absolute error is computed, providing a summary of the prediction error over time. By visualizing these mean errors, with error bars representing the standard deviation within each chunk, we aim to observe potential shifts in the distribution of prediction errors across different time periods. This approach allows us to examine how the model's performance may vary over time and identify any temporal distribution shifts in the prediction error.
    \begin{figure*}[t]
    \centering
    % \vspace{-1.2em}
    \includegraphics[width=0.45\textwidth]{figures/rebuttal/pem04_trend.pdf}
    \includegraphics[width=0.45\textwidth]{figures/rebuttal/pem08_trend.pdf}
    % \vspace{-1em}
    \caption{The mean absolute error per chronological chunk showing potential shifts in prediction accuracy over time for PeMS04 (Left) and PeMS08 (Right) datasets. Error bars represent the standard deviation within each chunk.}
    \label{fig:mae_distribution_shift}
    % \vspace{-1em}
    \end{figure*}
\end{itemize}

\subsection{Reviewer Vd3Z / Reviewer 3}
\begin{enumerate}
    \item \st{Inductive setting to accommodate new nodes.}
    \item Losing critical information due to the ignorance of non-linear interactions between node features. 
    \item Training time scalability with large graphs.
    \item \st{How to get positive weight in (5).}
    \item How does the narrowing the candidate nodes heuristic impact the ability to capture important node features. 
\end{enumerate}

\subsection{Summaries}

\begin{enumerate}
\item Asymptotic Training complexity / actual training time cost/ training time for large graph: R1 R3
\item Sensitivity analysis of K1 and K2, lambda 1 and lambda 2. Analysis  how the hyper-parameters influence the performance and time. Guideline of selecting K1 and K2, How does the narrowing the candidate nodes heuristic impact the ability to capture important node features: R1 R2 R3
\item Expressive power of SDGNN, theoretical or empirical: R2
\item Explain why SDGNN is better for the dynamic node feature scenario: R1.
\item Why the performance could be better than GNN. Visualize the embeddings?: R2
\item more discussion on limitation for non-linear interaction: R2, R3
\item Add experiments showing how performance degrades with increasing time gaps: R2\yhc{Mai TODO.}
\item Add memory requirement: R2
\item Add experiments on more diverse types of graph data beyond citation and traffic forecasting.: R2
\end{enumerate}

\section{Response Draft}

\subsection{Response to M5fg}

We sincerely appreciate your constructive and inspiring feedback.

{\bf Intuition of SDGNN.} Rather than inventing an efficient model with great performance, we aim to find a fundamental and model-agnostic solution to approximate the prediction of any target GNN model with efficient computation at the inference stage. Some recent GNN-MLP works like NOSMOG and VQGraph not only learn from the original target GNN model but also implicitly impose some additional modules to boost the performance. Therefore, they cannot be guaranteed to achieve performance similar to that of the stronger target GNNs, which is empirically verified in Table 2. Since we focus on approximating any target GNNs, we introduce additional flexibility in the sparse weights for a potentially powerful and universal structure to mimic the performance of ANY GNNs with efficient inference. We will add more elaborations to clarify the motivation in a revised version. 

{\bf Importance of components of SDGNN.} Both the structure and the optimization algorithm of SDGNN are critical to the performance. The SDGNN will not work without any of them. In the structure of SDGNN, the learnable feature transformation function and the sparse aggregation weights grant the model sufficient flexibility to approximate a wide range of target GNN models. The optimization algorithm actually finds the optimal learnable parameters. As for the inference time, the dominating factor is the number of non-zero entries in the sparse weight vectors, which is mainly controlled by the max LARS iterations. The performance will generally increase if we enlarge the max LARS iterations, but the improvement will quickly saturate once the max LARS iterations reach some threshold. $K_1$ and $K_2$ are hyper-parameters that shrink the search space of the LARS algorithm to reduce the training time. The training time will be shorter as the search space decreases, but the performance might drop if the candidate lacks sufficient critical neighbours. We will add more elaborations on the impact of the components of SDGNN in a revised version.

{\bf Significance of dynamic node features.} Besides the dynamic node features, SDGNN is also designed to handle the dependency on neighbour features. These features are valuable but challenging to achieve. First, some applications could benefit from such features. For example, the recent purchasing behaviour of one's closest friend might probably influence her online shopping preference; the traffic flow of an intersection in the near future should be correlated with the status of its neighbouring intersections, etc. Therefore, we want to develop a technique to efficiently summarize or approximate the dynamic and potentially critical neighbour features to fully convey the power of GNNs. Second, achieving these features simultaneously is challenging. Without dynamic node features, we always have an easy workaround method to cache all the predictions instead of cumbersome computation upon request. Without the critical dependency on neighbour features, the GNN-MLP approaches should work well. However, none of the existing methods can deal with the case where prediction could benefit from potentially dynamic node features, especially for those from a few critical neighbours. We will add more elaboration with examples to better convey the motivation of this work. 

{\bf Compare with VQGraph.} Thanks for bringing us the new GNN-MLP SOTA. We will add this reference in the related section in a revised version. Although this method reported better performance against other GNN-MLP methods like GLNN and NOSMOG, it does not impact the novelty of our work. First, like other GNN-MLP methods, VQGraph fully relies on the target node features, which cannot solve the case that the label could rely on the features of neighbour nodes. Second, VQGraph trains the target GNN with the coded node features and essentially implicitly changes the target GNN models, which could bring better or worse performance. As shown in Fig. 7 from the VQGraph paper, it does not consistently have improved performance with better target GNN models, while from Table 2, our method is designed to approximate the target GNN and consistently improves with better target GNN models. 

{\bf More experiments on heterophilic datasets.} We agree that adding more experiments on heterophilic datasets will strengthen our work. We believe the current experiments are sufficient to demonstrate the advantages of SDGNN. We will apply those experiments in future work. 

{\bf Asymptotic analysis.} The asymptotic convergence rate in terms of the number of iterations is very challenging due to the non-convex nature of the loss function and the stochastic characteristics of the training algorithm. As for the candidate node generation algorithm, we will generate it once and use the same set of candidates throughout the optimization. Therefore, it is not the dominating factor. For the LARS solver, the per-iteration complexity will be $|\mathbb{B}|(|\mathbb{C}_z|^3+|\mathbb{C}_z|^2d)$, where $|\mathbb{B}|$ is the batch size, $|\mathbb{C}_z|$ is the size of the candidate set and $d$ is the embedding dimension. We will add the complexity analysis in a revised version. 

{\bf Sensitivity Analysis.} $\lambda_2$ is a common hyper-parameter for the strength of L2 regularizor. $\lambda_1$ controls the sparsity. In our implementation, since we are using LARS, there is no explicit $\lambda_1$, and the sparsity is controlled via maximum LARS iteration. The performance will generally increase if we enlarge the max LARS iterations, but the improvement will quickly saturate once the max LARS iterations reach some threshold. As for $K_1$ and $K_2$, they jointly determine the size of the candidate node set. We attached a training curve for the Pubmed/SAGE case with different settings of $K_1$ with $K_2=0$ (see Fig. 3 in \url{https://docs.google.com/document/d/e/2PACX-1vRNHjyltQZUQs_IM0Ota0Zvm0eUO2PRbg1i-i02igGq9DsnIB3EANvRcn8w41R4NRN-b1JfqNnT2Ctw/pub}). Note that $K_1$ is the dominating factor for the size of the candidate and varying different $K_2$ will yield some intermediate results. We can see that the loss will converge faster with a small candidate size, but they will converge to some sub-optimal point. With a proper size ($K_1=3$ in this case), SDGNN will robustly and efficiently converge to some decent solution. We will add more elaborations on the impact of hyper-parameters and sensitivity experiments in the revised version. 

{\bf Training time/space cost.} We will add a detailed analysis of the time and space cost in a revised version. The time cost is indeed no cheaper than to train SAGE. The design of stochastic training and candidate pruning accommodates large-scale graphs, which helped us successfully train the SDGNN for the OGBN-Products in about 20 hours. Compared to GNNs like SAGE, the extra space cost comes from storing the sparse weights, which is proportional to the number of nodes and the number of non-zero entries of those weights. 

\subsection{Response to bvcp}

We thank you for your constructive and inspiring feedback.

{\bf Expressiveness of SDGNN.} We need to clarify that we aim to find a fundamental and model-agnostic solution to approximate the prediction of any target GNN model with efficient computation at the inference stage rather than inventing an efficient model with great performance. Therefore, the performance of SDGNN is designed to be similar to the target GNN models, which has been empirically demonstrated in Table 2 across extensive datasets and target GNN models. Other GNN-MLP works, such as NOSMOG, implicitly integrated additional modules to boost the performance of GNN (NOSMOG extend the distillation with augmented features), and that's why they could have potentially different performance than the target GNN. From Table 2, we can see that they will have better performance than a weak GNN target like SAGE (which is what they reported in their paper) but cannot achieve similar performance of stronger GNN models. 

Then, the question remains: under which condition can the SDGNN match the performance of a target GNN? This is really an interesting but challenging question, and we have not reached a complete answer for general cases. However, we have found some insights w.r.t. to a group of spectral GNN models. Inspired by the definitions in Sec. 2.2 of \citet{wang2022powerful}, we have found that the Filter-Most-Expressive GNNs can be well approximated via SDGNN with a theoretical guarantee. Specifically, it is defined as
\[
    \psi(\alpha(\mathbf{L})\varphi(\mathbf{X})),
\]
where $\mathbf{X}\in\mathbb{R}^{|\mathcal{V}|\times D}$ is the node feature matrix with $|\mathcal{V}|$ nodes and $D$ feature dimension, $\varphi(\cdot)$ and $\psi(\cdot)$ denotes MLPs operating on the rows of the input matrix, $\alpha(\cdot)$ denotes arbitrary real value filter function and $\mathbf{L}$ is the normalized graph Laplacian. This form covers a wide range of spectral GNNs (c.f. Appendix A from \citep{wang2022powerful}). 

Let's briefly analyze why SDGNN can cover the Filter-Most-Expressive GNNs. In SDGNN, if the downstream decoding function $f(\cdot)$ (in Sec. 6.1.5) is set to be $\psi(\cdot)$ and the feature transformation function $\phi(\cdot)$ is set to be $\varphi(\cdot)$, the $\mathbf{\theta}_z$ can be regarded as picking a few critical non-zero entries for the $z$th row of $\alpha(\mathbf{L})$ so that the result from SDGNN is as close as possible to the $z$th row of $\alpha(\mathbf{L})\varphi(\mathbf{X})$. A sufficient condition would be that $\|\alpha(\mathbf{L})- \mathbf{\Theta}\circ\alpha(\mathbf{L})\|_2$ is small where $\|\cdot\|_2$ denotes the spectral norm and $\circ$ denotes the element-wise product operation. \citet{bhattacharjee2024universal} indicates that for any positive number $\epsilon>0$, there exists a $\mathbf{\Theta}$ with $O(|\mathcal{V}|/\epsilon^2)$ non-zero entries, such that $\|\alpha(\mathbf{L})- \mathbf{\Theta}\circ\alpha(\mathbf{L})\|_2\le\epsilon|\mathcal{V}|$ if $\alpha(\mathbf{L})$ is positive semidefinite. For general $\alpha(\mathbf{L})$, it satisfies that $\|\alpha(\mathbf{L})- \mathbf{\Theta}\circ\alpha(\mathbf{L})\|_2\le\epsilon~\text{max}(|\mathcal{V}|, \|\alpha(\mathbf{L})\|_1)$, where $\|\cdot\|_1$ denotes the nuclear norm. 

These facts indicate that SDGNN can well approximate the Filter-Most-Expressive GNNs, which cover a wide range of popular spectral GNNs. We will add this analysis in a revised version. 

{\bf Performance gap with increasing time gaps.} We have included extra results for this purpose in Fig. 1 and Fig. 2 in \url{https://docs.google.com/document/d/e/2PACX-1vRNHjyltQZUQs_IM0Ota0Zvm0eUO2PRbg1i-i02igGq9DsnIB3EANvRcn8w41R4NRN-b1JfqNnT2Ctw/pub}. We plot the absolute error with standard deviation from 10 equal-sized chunks split by time. We can see that the performance will be worse when time gaps are larger from the training set. 

{\bf Memory requirement.} We will replace Table 2 with the following table with memory requirements. All method requires $O(|\mathcal{V}|D)$ to store the node features. Besides, SDGNN requires extra space of $O(|\mathcal{V}|\bar{d}L)$ to store the sparse weights, which have a similar size to the node features in the empirical results. 

\yhc{Remember to add the actual table here.}

{\bf Handling the Distribution shift.} A typical and practical solution is periodically retraining new models based on recently collected data. This can solve the distribution shift issue for both the target GNN model and SDGNN. If we trade the performance for less computation overhead, we can periodically and partially update SDGNN for better training efficiency. For example, we can keep the weight matrix $\mathbf{W}$ unchanged and only periodically perform a Phase $\mathbf{\Theta}$ update according to the latest data. A fundamental approach could incorporate online learning so that the trainable weights from the target GNN and SDGNN can be adapted as more data become available and the graph topology changes. However, developing such a method is involved due to the challenges of enforcing a sparse solution. We would leave this as a future work. We will add more details in a revised version. 

{\bf More experiments on diverse datasets.} We agree that adding more experiments will strengthen our work. We believe the current experiments are sufficient to demonstrate the advantages of SDGNN. Note that the OGBN-Products dataset is not from a citation network but is large-scale, well-accepted and challenging data from the Amazon product co-purchasing network. We want to leave the discussion for more diverse datasets in some future works. 

{\bf Guideline to select $K_1$ and $K_2$.} We don't have a general optimal method for selecting these parameters. The strategy we were adopting was to set them to make the size of the candidate nodes similar to or slightly larger than the size of receptive nodes from the target GNN models. Specifically, We first set $K_1$ according to this criterion with $K_2=0$. Then, we add more nodes by searching $K_2$ with different positive numbers. 

{\bf Theoretical analysis.} Please refer to the response in the expressiveness of GNN. 

{\bf Non-linear interactions between node features.} From the analysis for expressiveness, SDGNN can well approximate the Filter-Most-Expressive GNNs, which cover lots of well-known GNNs. We will add more arguments for the non-linear feature interaction issue. For theoretical analysis on a more general case, we will leave it to future work. 

{\bf Handling new nodes in the inductive setting.} I should admit that I don't have a principled approach to solving this issue with the current algorithm. A simple engineering strategy to handle the novel nodes in real-time could be collecting the $\mathbf{\theta}$ for all/sampled $1$-hop neighbour nodes and summing them up as the proxy for the new nodes. Moreover, for the situation where we are allowed to do some preprocessing for the novel nodes, we could use the inductive GNN to infer the GNN embedding, compute $\mathbf{\theta}$ with Phase $\mathbf{\theta}$ for that node and cache it. Then, the actual online inference stage will be the same as the other nodes that are seen during the training of SDGNN. We will add more elaboration in a revised version. 

\subsection{Response to Vd3Z}

Thank you for your constructive and inspiring feedback on our work. 

{\bf Handling new nodes in the inductive setting.} We need to clarify that our method pre-computes the optimal and sparse aggregation weights over a few nodes rather than the ``embeddings'' for all nodes. We admit that our method was not designed to handle the new nodes in a principled way. In the appendix, we pointed it out in Sec. D.1 that some native engineering approaches can process the new nodes. A simple strategy could be collecting the $\mathbf{\theta}$ for all/sampled $1$-hop neighbour nodes and summing them up as the proxy for the new nodes. Moreover, for the situation where we are allowed to do some preprocessing for the novel nodes, we could use the inductive GNN to infer the GNN embedding, compute $\mathbf{\theta}$ with Phase $\mathbf{\theta}$ for that node and cache it. Then, the actual online inference stage will be the same as the other nodes that are seen during the training of SDGNN. We will add more elaboration in a revised version. 

{\bf Non-linear interactions.} We don't have the complete answer for the general GNNs, but we have found some theoretical guarantees for a group of GNN models. Inspired by the definitions in Sec. 2.2 of \citet{wang2022powerful}, we have found that SDGNN has sufficient expressive power to approximate the Filter-Most-Expressive GNNs without the risk of losing important non-linear interactions between node features. Specifically, it is defined as
\[
    \psi(\alpha(\mathbf{L})\varphi(\mathbf{X})),
\]
where $\mathbf{X}\in\mathbb{R}^{|\mathcal{V}|\times D}$ is the node feature matrix with $|\mathcal{V}|$ nodes and $D$ feature dimension, $\varphi(\cdot)$ and $\psi(\cdot)$ denotes MLPs operating on the rows of the input matrix, $\alpha(\cdot)$ denotes arbitrary real value filter function and $\mathbf{L}$ is the normalized graph Laplacian. This form covers a wide range of spectral GNNs (c.f. Appendix A from \citep{wang2022powerful}). 

Let's briefly analyze why SDGNN can cover the Filter-Most-Expressive GNNs. In SDGNN, if the downstream decoding function $f(\cdot)$ (in Sec. 6.1.5) is set to be $\psi(\cdot)$ and the feature transformation function $\phi(\cdot)$ is set to be $\varphi(\cdot)$, the $\mathbf{\theta}_z$ can be regarded as picking a few critical non-zero entries for the $z$th row of $\alpha(\mathbf{L})$ so that the result from SDGNN is as close as possible to the $z$th row of $\alpha(\mathbf{L})\varphi(\mathbf{X})$. A sufficient condition would be that $\|\alpha(\mathbf{L})- \mathbf{\Theta}\circ\alpha(\mathbf{L})\|_2$ is small where $\|\cdot\|_2$ denotes the spectral norm and $\circ$ denotes the element-wise product operation. \citet{bhattacharjee2024universal} indicates that for any positive number $\epsilon>0$, there exists a $\mathbf{\Theta}$ with $O(|\mathcal{V}|/\epsilon^2)$ non-zero entries, such that $\|\alpha(\mathbf{L})- \mathbf{\Theta}\circ\alpha(\mathbf{L})\|_2\le\epsilon|\mathcal{V}|$ if $\alpha(\mathbf{L})$ is positive semidefinite. For general $\alpha(\mathbf{L})$, it satisfies that $\|\alpha(\mathbf{L})- \mathbf{\Theta}\circ\alpha(\mathbf{L})\|_2\le\epsilon~\text{max}(|\mathcal{V}|, \|\alpha(\mathbf{L})\|_1)$, where $\|\cdot\|_1$ denotes the nuclear norm. 

These facts indicate that SDGNN can well approximate the Filter-Most-Expressive GNNs without the issue of losing important non-linear interactions. For more general cases, we will leave the theoretical analysis in future work. We will add this analysis in a revised version.

{\bf Scalability.} The structure of SDGNN guarantees low inference computation complexity, while the mini-batch training and candidate narrowing strategy makes the training of SDGNN scale to large graphs. 

The inference computation complexity is proportional to the number of receptive nodes, which is the number of non-zero entries in the sparse weight vector in SDGNN. The sparsity is guaranteed via the optimization algorithm. 

For the training time, the mini-batch sampling and narrowing of the candidate node sets make the per-iteration complexity scalable to large graphs. Specifically, mini-batch sampling makes each iteration's cost proportional to the batch size rather than the size of the graph. Within the LARS solver, the candidate selection strategy further reduces the complexity into $(|\mathbb{C}_z|^3+|\mathbb{C}_z|^2d)$ for each node, where $|\mathbb{C}|$ is the size of the candidate nodes and $d$ is the embedding size, which is independent of the graph size. Along with the Phase $\mathbf{W}$, the per-iteration complexity is $O(|\mathbb{B}|(k(Dd+L^\prime d^2) + |\mathbb{C}_z|^3+|\mathbb{C}_z|^2d))$, where $L^\prime$ is the number of layers in the feature transformation function and $k$ is the SGD iterations for Phase $\mathbf{W}$. We can see that per-iteration complexity is independent of the size of the graph.

We have also demonstrated the scalability with the OGBN-products dataset, which is a well-known large-scale dataset with 2.4 million nodes. The training takes about 20 hours, and Figure 2 depicts that the inference complexity is much lower than the target GNN models. 

{\bf How to enforce the non-negative condition in (5).} The Least Angle Regression algorithm implemented in the Scikit-learn package has a built-in option of it. We will provide some details about this in a revised version. 

{\bf Impact of narrowing the candidate nodes.} We don't have a complete theoretical guarantee for this procedure, but the rule of thumb is to set them to make the size of the candidate nodes similar to or slightly larger than the size of receptive nodes from the target GNN models. We attached a training curve for the Pubmed/SAGE case with different settings of $K_1$ with $K_2=0$ (see Fig. 3 in \url{https://docs.google.com/document/d/e/2PACX-1vRNHjyltQZUQs_IM0Ota0Zvm0eUO2PRbg1i-i02igGq9DsnIB3EANvRcn8w41R4NRN-b1JfqNnT2Ctw/pub}). Note that $K_1$ is the dominating factor for the size of the candidate and varying different $K_2$ will yield some intermediate results. We can see that the overly shrunk candidate set will result in sub-optimal performance. In practice, we need some hyper-parameter search to strike a balance between the training complexity and the overall performance. We will add more elaborations for this issue in a revised version.


==> sections/tables/performance_compare.tex <==
%!TEX root = /Users/yaochen/Dropbox/Apps/Overleaf/AAAI25-SDGNN/main.tex
\begin{table}[t]
\centering
\caption{Asymptotic complexity for different approaches for online prediction of GNN. $D$: average node degree; $d$: dimension of node embedding of GNN models; $c$: size of the dictionary; $F$: node feature dimension; $s$: average number of non-zero elements per row of the dictionary; $n_a$: average number of non-zero elements of $\va$; $S$: neighbor sampling size; $L$ number of layer in GNN.}
% \vspace{1mm}
\label{tab:compare}
% \hspace{-20mm}
\begin{tabular}{llllll}
\hline
Approach   & Latency & Preprocess Time & Extra Memory                             \\ \hline
Vanilla    & $O(D^LF)$          & None                 & None                                    \\
GraphSAGE  & $O(S^LF)$         & None                  & None                                    \\
GAMLP      & $O(1)$             & $O(D|\gV|LF)$        & $O(|\gV|d)$                                \\
SDMP(ours) & $O(nF)$            & $O(csF)$           & $O(2|\gV|n_a+cF)$   \\ \hline
\end{tabular}
\end{table}
% For extra memory, the current version did not consider the A^K in GAMLP and O in SDMP. O should be generally smaller than A^K, which is a fair comparation. 
